The Price of Incentivizing Exploration: A Characterization via Thompson Sampling and Sample Complexity

We consider incentivized exploration: a version of multi-armed bandits where the choice of arms is controlled by self-interested agents, and the algorithm can only issue recommendations. The algorithm controls the flow of information, and the information asymmetry can incentivize the agents to explore. Prior work achieves optimal regret rates up to multiplicative factors that become arbitrarily large depending on the Bayesian priors, and scale exponentially in the number of arms. A more basic problem of sampling each arm once runs into similar factors. We focus on the price of incentives: the loss in performance, broadly construed, incurred for the sake of incentive-compatibility. We prove that Thompson Sampling, a standard bandit algorithm, is incentive-compatible if initialized with sufficiently many data points. The performance loss due to incentives is therefore limited to the initial rounds when these data points are collected. The problem is largely reduced to that of sample complexity: how many rounds are needed? We address this question, providing matching upper and lower bounds and instantiating them in various corollaries. Typically, the optimal sample complexity is polynomial in the number of arms and exponential in the "strength of beliefs".

==> abstract.tex <==
We consider \emph{incentivized exploration}: a version of multi-armed bandits where the choice of arms is controlled by self-interested agents, and the algorithm can only issue recommendations. The algorithm controls the flow of information, and the information asymmetry can incentivize the agents to explore. Prior work achieves  optimal regret rates up to multiplicative factors that become arbitrarily large depending on the Bayesian priors, and scale exponentially in the number of arms. A more basic problem of sampling each arm once runs into similar factors.

We focus on the \emph{price of incentives}: the loss in performance, broadly construed, incurred for the sake of incentive-compatibility. We prove that Thompson Sampling, a standard bandit algorithm, is incentive-compatible if initialized with sufficiently many data points. The performance loss due to incentives is therefore limited to the initial rounds when these data points are collected. The problem is largely reduced to that of sample complexity: how many rounds are needed? We address this question, providing matching upper and lower bounds  and instantiating them in various corollaries. Typically, the optimal sample complexity is polynomial in the number of arms and exponential in the ``strength of beliefs".



==> explorability.tex <==

\section{Explorability}

Here we fully characterize the set of explorable arms in the independent. We give a similar statement for the dependent case but do not determine the precise statement for edge cases in which some explorations are BIC with no margin.  \cite{SyrgkanisCB-2016} gives a complete but more abstract characterization which subsumes these results but our statements are more explicit. Moreover our proof in the independent case is simple and self-contained while our proof in the dependent case motivates the minimax procedure we use to obtain a sample-efficient exploration algorithm.

\begin{lemma}

Assume that in the prior, the $K$ arms have independent rewards with prior means $1>\mu_1^0\geq \mu_2^0\geq \dots\geq \mu_K^0>0$. Suppose that the infimal possible values of the true means are $m_1,\dots,m_K$. Define the increasing sequence $n_j=\max_{i\leq j} m_i$. Let $j$ be such that $\mu_{j+1}^0 \leq n_j$ for the first time. Then arms $a_1,\dots,a_j$ are explorable arbitrarily many times. The only other potentially explorable arms are those $a_k$ with $\mu_k^0=n_j$. Let $S=\{i\leq j:m_i=n_j\}$ and $R=\{k:\mu_k^0=n_j\}$. These additional arms $a_k$ for $k\in R$ are explorable with positive probability if and only if for all $i\in S$, the prior distribution of $\mu_i$ is supported inside the two point set $\{m_i,1\}$, and moreover the true value of $\mu_i$ is $m_i$. If $k\in R$ has $\mu_k$ almost surely constant, then $a_k$ is explorable exactly on the event $E$ that $\mu_i=n_j$ for all $i\in S$. If $k\in R$ does not has $\mu_k$ almost surely constant, then $a_k$ is explorable no matter what the true arm means are.

\end{lemma}

\begin{proof}

We first argue that arms $a_1,\dots, a_j$ are explorable. We argue inductively, so we suppose that arms $a_1,\dots,a_i$ are explorable arbitrary many times. The point is that by independence, for any $\varepsilon>0$ for some large $t$ with positive probability we have

\[\mathbb E[\mu_k|\mathcal F_t]\leq m_i+\varepsilon\]

for all $k\leq i$. Indeed, we have $\mu_k\leq m_i+2\varepsilon$ with positive probability and the conditional expectation $\mathbb E[\mu_k|\mathcal F_t]$ converges to $\mu_k$ in $L^1$ as the number of samples of $\mu_k$ tends to infinity. If $a_{i+1}$ has not yet been explored, then it can be in such a situation by taking $\varepsilon$ sufficiently small. Moreover, by using the lemmas of section 2 we can use this leverage to explore arm $a_{i+1}$ arbitrarily many times with probability $1$.

On the other hand, if $\mu_k^0<n_j$ then $a_k$ is never explorable. Indeed, for sake of contradiction let $t$ be the first time at which $a_k$ is explored with positive probability by a BIC algorithm, then we have $\mathbb E^t[\mu_k]=\mu_k^0<\mathbb E^t[\mu_i]$ where $m_i=n_j$.

For the edge-case arms with $\mu_k^0=n_j$ we use a similar argument. Again take $i$ with $m_i=n_j$ and observe that unless $\mu_i\in \{m_i,1\}$ with probability $1$, we will have $\mathbb E[\mu_i|\mathcal F_t]>m_i$ with probability $1$ for all times $t$. Therefore by the same argument as in the previous paragraph, arms $a_k$ with $\mu_k^0=n_j$ are not explorable unless this property holds for all $i\in S$. Now suppose we do have $\mu_i\in \{m_i,1\}$ with probability $1$ for all $i\in S$. Then we still have $\mathbb E[\mu_i|\mathcal F_t]\geq m_i$ with probability $1$ for all $t$, which means that the first attempted exploration of arm $a_k$ is only BIC if $\mathbb P^t[\mu_i=m_i]=1.$ This is of course only possible when $\mu_i=m_t$. Conversely, if $\mathbb P^0[\mu_i\in\{m_i,1\}=1$ and $\mu_i=m_i$ then we will have $\mathbb P^t[\mu_i=m_i]=1$ for sufficiently large $t$ by sufficient exploration of $a_i$.

In the case that $\mu_k=\mu_k^0$ almost surely for some $k\in R$, it is clear that $a_k$ is explorable exactly on the event that $\mu_i=n_j$ for all $i\in S$, as exploring it once conveys no additional information so it is equivalent to exploring for the first time. On the other hand if $\mu_k$ has any uncertainty, then we explain how to explore $a_k$ with probability $1$. In the event that $E$ holds, let $t$ be a fixed time such that $a_k$ has been explored with positive probability by time $t$. Then consider the partial strategy which at time $t+1$ explores $a_k$ with probability $1$ if its first sample gave a reward. This is $(k,\alpha)$-BIC for some positive $\alpha$, and therefore there is a BIC strategy which explores with positive probability $\Omega(\alpha)$ at time $t+1$ regardless of the history. Doing this $O(\alpha^{-1})$ times with coupled randomness allows us to explore $a_k$ almost surely by time $t+O(\alpha^{-1})$.

\end{proof}

We also give a version of the above for dependent arms, which can be viewed as a motivation for the minimax analysis used for exploration. We do not give the corresponding edge case as it seems more complicated to state and should in principle be subsumed in the work \cite{SyrgkanisCB-2016}.


\begin{theorem}
\label{thm:explorable}
The set $S_*$ of explorable actions contains the result of the following iterative construction: start with $S$ containing only the arm with highest prior mean, and add arm $a_k$ to $S$ if for every $q\in \Delta_K$ we have

\[\min_{q\in \Delta_K}\mathbb E\bigg[\mathbb E[\mu_k-\mu_q|\{\mu_{s}\forall s\in S\}]_+  \bigg]>0.\]

At the end, set $S_*=S$.

\end{theorem}


\begin{proof}

First, let us assume that arm rewards are deterministic instead of stochastic, so the planner knows the conditional expectations $\mathbb E[\mu_j|\{\mu_s\forall s\in S\}]$ exactly for all $j\in [K]$. We suppose that $S$ is explorable and prove that arms $a_k$ as defined above are also explorable. Consider the two-player asymmetric-information zero-sum game defined as follows. The planner knows $\{\mu_s|s\in S\}$ while the planner knows nothing. The planner and agent each simultaneously choose an arm: the planner chooses from $S\cup\{a_k\}$ while the agent chooses from $[K]$. If the planner chooses arm $a_k$ and the agent chooses arm $a_j$, then the planner's payoff is $\mu_i-\mu_j$. If the planner chooses arm $a_s$ for $s\in S$ then the payoff is $0$.\\

By the minimax theorem, the game's value is unchanged if either player reveals his strategy profile first. When the agent reveals first, by initial assumption the game has value at least \[\min_{q\in\Delta_K}\mathbb E\bigg[\mathbb E[\mu_k-\mu_q|\{\mu_{s}\forall s\in S\}]_+  \bigg]>0.\]

When the planner reveals first, he has a strategy with the same value. By definition this strategy, modified to play myopically if not playing arm $a_k$, is a BIC strategy which recommends arm $k$ a positive fraction of the time. Therefore we have proved the theorem in the deterministic rewards case.\\

When rewards are random, by standard martingale theory, conditional expectations of arm means converge to the truth in $L^1$ given a sufficiently large but fixed sample size. When we have an $L^1$ approximation smaller than the value of the game we can invoke the deterministic case to solve the randomized case. (Here we use the strictness of the inequality in the Theorem statement.) 


\end{proof}

==> frequentist_regret.tex <==


\section{Frequentist Regret with Artificial Priors}

Here we expand on the work \cite{Shipra-aistats13} which gives tight regret bounds for Thompson sampling initialized with i.i.d. uniform and Gaussian priors. Their main result for Beta priors is:

\begin{theorem}
\label{thm:agrawalgoyal}
Thompson sampling with Beta priors has problem-dependent expected regret

\begin{equation}\label{eq:TSfreqgap}\mathbb{E}[R(T)] \leq(1+\epsilon) \sum_{i=2}^{K} \frac{\log T}{d\left(\mu_{i}, \mu_{1}\right)} \Delta_{i}+O_{\vec\mu}\left(\frac{K}{\epsilon^{2}}\right)\end{equation}

and problem-independent expected regret

\begin{equation}\label{eq:TSfreqnogap} \leq O(\sqrt{KT\log(T)}).\end{equation}

Here $d\left(\mu_{i}, \mu_{1}\right):=\mu_{i} \log \frac{\mu_{i}}{\mu_{1}}+\left(1-\mu_{i}\right) \log \frac{\left(1-\mu_{i}\right)}{\left(1-\mu_{1}\right)}$ is the KL divergence.

\end{theorem}

We investigate the effect of an artificial informative Beta prior on the frequentist minimax regret of Thompson sampling. We view informative Beta priors as a natural setting for our results to be applied, as it allows for incorporation of public information. Call a Beta prior $M$-informative if it includes at most $M$ fake samples per arm, and optimistic if it includes only positive information on the arms.

Our results are as follows. First, when the gap size is large, we show that an $M$-informative prior obeys the regret bound of Equation~\ref{eq:TSfreqgap} up to an additive $2^{O(M)}$ error term, which is necessary. On the other hand we give examples in which Thompson sampling suffers regret $\Omega(T^{1-\frac{1}{M}})$ when the gaps can be small. These examples require the best arm to be almost perfect, and we suspect that a more careful analysis would yield much better positive results when the best arm probability is bounded away from $1$. We also show that optimistic priors have very mild additive $M$-dependence. Finally, we show that these bounds hold even with additional and adaptive free-but-adversarial exploration. This means that in analyzing the frequentist regret of our BIC algorithm, it suffices to apply the bounds we give here to the initialized prior and add the number of initial exploration steps.

To prove these results, we adapt Lemmas 2.8-2.12 of their paper. Lemmas 2.8 and 2.12 are entirely unchanged, and Lemma 2.10 follows from plugging into Lemma 2.9. So we focus on Lemmas 2.9 and 2.11. Their regret is decomposed into a sum of three terms, and Lemmas 2.9 and 2.11 each correspond to one of these terms. 

We recall some notations and definitions from that paper:

\begin{lemma}

For $M$-informative priors we have

\[\mathbb E^M\left[\frac{1}{p_{i,\tau_k+1}}-1\right]\leq \frac{a_{k,i}}{(1-\mu)^M}.\]

Here $a_{k,i}$ is the $M=0$ upper bound given by

\[a_{k,i}=\left\{\begin{array}{ll}
\frac{3}{\Delta_{i}'} \text { for } k<\frac{8}{\Delta_{i}^{\prime}} & \\
\Theta\left(e^{-(\Delta'_{i})^{2} k / 2}+\frac{1}{(k+1) \Delta_{i}^{\prime 2}} e^{-D_{i} k}+\frac{1}{e^{\Delta_{i}^{\prime 2} k / 4}-1}\right) \text { for } k \geq \frac{8}{\Delta_{i}^{\prime}}
\end{array}\right.\]

Moreover for optimistic priors we have the original upper bound of $a_{k,i}$.

\end{lemma}

\begin{proof}

Since $\frac{1}{p_{i,\tau_k+1}}-1$ is a positive function, and any $M$ initial string of samples would have probability $2^{-O_{\mu}(M)}$ of happening initially anyway, the result follows. In the optimistic case, clearly $p_{i,\tau_k+1}$ will stochastically increase so the expectation considered will decrease.

\end{proof}

\begin{lemma}

We have 

\[\sum_k \mathbb E^M\left[\frac{1}{p_{i,\tau_k+1}}-1\right]\leq 2^{O_{\mu}(1)}.\]

Here $O_{\mu}(1)$ tends to infinity as $\mu\to 1$.

\end{lemma}

\begin{proof}

It is a geometrically decaying series past $k\geq O(\Delta_i^{-2}).$

\end{proof}

Now we give a tighter bound.

\begin{lemma}

For any positive integer $n$ and $k\geq n\left(\mu-\mu(1-\mu)\varepsilon\right)$ we have

\[\frac{\mathbb P[Bin(n,\mu)=k]}{\mathbb P[Bin(n,\mu)=k+1]}\geq 1-\varepsilon.\]

\end{lemma}

\begin{proof}

The ratio is 

\[\frac{\binom{n}{k}(1-\mu)}{\binom{n}{k+1}\mu}=\frac{1-\mu}{\mu}\frac{k+1}{n-k}\geq \frac{(1-\mu)k}{\mu(n-k)}.\]

Plugging in $k\geq n\left(\mu-\mu(1-\mu)\varepsilon\right)$, the RHS becomes

\begin{align}\frac{(1-\mu)k}{\mu(n-k)} &= \frac{1-\mu}{\mu} \cdot\frac{\mu(1-(1-\mu)\varepsilon)}{(1-\mu)(1+\mu\varepsilon)}\\
&=\frac{1-(1-\mu)\varepsilon}{1+\mu\varepsilon}\\
&\geq (1-(1-\mu)\varepsilon)\cdot (1-\mu\varepsilon)\\
&\geq 1-\varepsilon.
\end{align}

\end{proof}

\begin{lemma}

For $M$-informative priors and $M'\geq \frac{1000 M^2\log(T)\mu}{1-\mu}$ we have 

\[\mathbb E^M\left[\min\left(\frac{1}{p_{i,\tau_k+1}}-1,T\right)\right]\leq T^{-9}+3a_{M'+M}.\]

\end{lemma}

\begin{proof}



For $k\geq M'\left(\mu-\mu(1-\mu)\varepsilon\right)$ we have for any $L\leq M$:

\[\frac{\mathbb P[Bin(M,\mu)=k]}{\mathbb P[Bin(M,\mu)=k+L]}\geq (1-\varepsilon)^M\geq  1-M\varepsilon.\]

Next, we have $\mathbb P[Bin(M,\mu)\leq M\mu+1]\geq \frac{1}{2}.$ This implies

\[\mathbb P[Bin(M+M',\mu)= k] \geq \frac{1}{2}\cdot \min_{0\leq L\leq  M\mu+1} \mathbb P[Bin(M',\mu)=k-L].\]

Using this we obtain, for any $k\geq M'\left(\mu-\mu(1-\mu)\varepsilon\right)+M\mu+1$:

\begin{align}
\frac{\mathbb P[Bin(M+M',\mu)= k]}{\mathbb P[Bin(M',\mu)= k]}&\geq \frac{\min_{0\leq L\leq  M\mu+1} \mathbb P[Bin(M',\mu)=k-L]}{2\cdot \mathbb P[Bin(M',\mu)= k]}\\
&\geq \frac{1-(M\mu+1)\varepsilon}{2}.
\end{align}

On the other hand, Bennett's inequality implies that 

\[\mathbb P\left[Bin(M',\mu)\leq M'\mu-10M'\mu(1-\mu)\varepsilon\right]\leq \exp\left(-M'\mu(1-\mu)\varepsilon^2\right). \]

Suppose that $M'\geq \frac{1000 M^2\log(T)\mu}{1-\mu}$ and take $\varepsilon=\frac{1}{10M\mu}.$ Then we have

\[M'\mu(1-\mu)\varepsilon = 100 M\log(T) \geq M\mu+1.\]

Then the above derivations show that for any \[k\geq M'\left(\mu-\mu(1-\mu)\varepsilon\right)+M\mu+1\geq M'\mu-\frac{M'(1-\mu)}{10M}\]

we have

\[\frac{\mathbb P[Bin(M+M',\mu)= k]}{\mathbb P[Bin(M',\mu)= k]}\geq \frac{1}{3}.\]

while Bennett's inequality specializes to:

\[\mathbb P\left[Bin(M',\mu)\leq M'\mu-\frac{M'(1-\mu)}{10M}\right]\leq T^{-10}.\]

Now let $q_{M'}(m)=\min\left(\frac{1}{p_{i,\tau_{M'+M}}(m)}-1,T\right)$. Then for an $M$-informative prior and $M'\geq \frac{1000 M^2\log(T)\mu}{1-\mu}$ we have

\begin{align}\mathbb E^{m\sim Bin(M',\mu)}[q_{M'}(m)]&=\sum_{m\leq M+M'} \mathbb P[Bin(M',\mu)=m]\cdot q_{M'}(m)\\
&\leq T^{-9}+ \sum_{M'\mu-\frac{M'(1-\mu)}{10M}\leq m\leq M+M'} \mathbb P[Bin(M',\mu)=m]\cdot q_{M'}(m)\\
&\leq T^{-9}+3\cdot \sum_{M'\mu-\frac{M'(1-\mu)}{10M}\leq m\leq M+M'} \mathbb P[Bin(M'+M,\mu)=m]\cdot q_{M'}(m)\\
&\leq T^{-9}+3\cdot\mathbb E^{m\sim Bin(M'+M,\mu)}[q_{M'}(m)]\\
&=T^{-9}+3a_{M'+M}.
\end{align} 

\end{proof}

\begin{lemma}

We have

\[\sum_{k\geq 1} \mathbb E[q_k]\leq \frac{10000M^2\log(T)\mu+M}{\Delta(1-\mu)^{M+1}}+T^{-8}+3\sum_{j\geq 1} a_{j}.\]

\end{lemma}

\begin{proof}

Follows from the previous lemma.

\end{proof}

\begin{lemma}

For $M$-informative priors we have

\[\sum_{t\leq T} \mathbb P[i(t)=i,\overline{E_i^{\mu}(t)}]\leq \left(\frac{M}{x_i-\mu_i}+\frac{1}{(x_i-\mu_i)^2}\right)\]

and also 

\[\sum_{t\leq T} \mathbb P[i(t)=i,\overline{E_i^{\mu}(t)}]\leq O_{\mu}\left(\frac{M}{\delta(x_i-\mu_i)}\right)+\frac{1}{d(x_i-\delta,\mu_i)}.\]

Moreover for pessimistic priors, we have the $M=0$ bound

\[\sum_{t\leq T} \mathbb P[i(t)=i,\overline{E_i^{\mu}(t)}]\leq 1+\frac{1}{d(x_i,\mu_i)}.\]

\end{lemma}

\begin{proof}

The proof of Agrawal and Goyal goes by upper bounding the LHS by the expected function of times that $\hat\mu_i\geq x_i$. In the pessimistic case this bound certainly can only improve.

In the general case, we observe that after $O\left(\frac{M}{x_i-\mu_i}\right)$ samples, having $\hat\mu_i\geq x_i$ implies having the empirical average of the real samples larger than $x_i-\delta>\mu_i$ for $\delta=\frac{x_i-\mu_i}{2}$. Now applying the $M=0$ bound and using Pinsker for all times past the first $O\left(\frac{M}{x_i-\mu_i}\right)$ then gives first claim. Taking $\delta$ small similarly implies the second.

\end{proof}

\begin{theorem}

Using $M$-informative Beta priors, we have

\[\mathbb E^M[R(T)] \leq 2^{O_{\mu}(M)}+(1+\epsilon) \sum_{i\neq i^*} \frac{\Delta_{i}\log T}{d\left(\mu_{i}, \mu_{i^*}\right)} +O_{\vec\mu}\left(\frac{K}{\epsilon^{2}}\right).\]

Moreover for $M$-optimistic Beta priors

\[\mathbb E^M[R(T)]\leq O(KM)+O\left(\sum_{i\neq i^*} \frac{\Delta_{i}\log T}{d\left(\mu_{i}, \mu_{i^*}\right)}\right) +O_{\vec\mu}\left(\frac{K}{\epsilon^{2}}\right).\]

Moreover there exist $L$-informative priors with $\mu_1-\mu_2\geq 0.1$ and expected regret $\Omega(2^L)$ after $T=2^L$ time-steps.

\end{theorem}



\begin{proof}

For the last part, we consider the following initialization with two arms:

\[(\mu_1,\mu_2)=(0.9,0.8)\]

with priors $\mu_1\sim Beta(1,M+1)$ and $\mu_2\sim Beta(M+1,1)$. In this case, with positive probability, the subjective expectation of $\mu_2$ will stay above $0.7$ for all time, and so $\mathbb P[\theta_2(t)<0.5]$ will decay exponentially with $t$. Hence with uniformly positive probability, $\theta_2(t)\geq 0.5$ for all $t$ simultaneously.

On this event, we can only sample arm $a_1$ if $\theta_1(t)\geq 0.5$. This has probability exponentially small in $L$ until the first time $a_1$ is sampled, hence takes an exponentially long time to occur on average, leading to exponential in $L$ regret.

In the other direction, we explain modifications of Lemmas 2.9 and 2.11 in Agrawal and Goyal.

Lemma 2.11 of Agrawal and Goyal states that when $M=0$, for $i\neq 1$ we have

\[\sum_{t=1}^{T} \operatorname{Pr}(i(t)=i, \overline{E_{i}^{\mu}(t)}) \leq \frac{1}{d\left(x_{i}, \mu_{i}\right)}+1.\]

The analog, our Lemma~\ref{lem:2.11} incurs an additive $O(M)$ cost in the regret, as well as an $O(1)$ multiplicative factor. Since this term only contributes to the $O_{\mu}(\varepsilon^{-2})$ of the regret bound, this is fine.

Lemma 2.9 is where the upper bound takes on an additional additive $2^{O_{\mu}(M)}$. Note that as we saw before there is no additional contribution for optimistic priors, which establishes the second assertion of the Theorem. In general, the regret has an additive term

\[\sum_{k\geq 0} \mathbb E\left[\frac{1}{p_{i,\tau_k+1}}-1\right].\]

We previously established that this was $2^{O_{\mu}(M)}$. The final regret bound is just obtained by summing these terms. So we see that the change is an additive $2^{O_{\mu}(M)}$ as claimed.

\end{proof}


Now we show that the situation is much worse with minimax regret, but only in the presence of a nearly perfect arm.

\begin{lemma}

If $\theta_1\sim Beta(1,M+1)$ and $\theta_2\sim Beta(a,b)$ then $\mathbb P[\theta_1\geq \theta_2] = \frac{(M+1)(a+b-1)!(M+b-1)!}{(b-1)!(M+a+b-1)!}.$

\end{lemma}

\begin{proof}

We integrate over the density of $\theta_2$ and the CDF of $\theta_1$ and use the standard value of the Beta integral to find

\begin{align}\mathbb P[\theta_2(t)\leq\theta_1(t)]&=(M+1)\frac{(a+b-1)!}{(a-1)!(b-1)!}\int_0^1 (1-x)^M x^{a-1}(1-x)^{b-1}dx\\
&=(M+1)\frac{(a+b-1)!}{(a-1)!(b-1)!} \frac{(M+b-1)!(a-1)!}{(M+a+b-1)!} \\
&= \frac{(M+1)(a+b-1)!(M+b-1)!}{(b-1)!(M+a+b-1)!}.   \end{align}

\end{proof}

\begin{theorem}



For fixed $M\geq 1$ and large $T$, it is possible for Thompson sampling with $M$-informative pessimistic Beta priors to have $\mu_{i^*}=1-T^{-\frac{1}{M}}$ and expected regret $\Omega_M(T^{1-\frac{1}{M}}).$ However we also have the upper bound

\[\mathbb E^M[R(T)] \leq O\left(\sqrt{KT\log(T)}\right)+O\left(\frac{KM^2\log(T)\mu+KM}{(1-\mu_{i^*})^{M+1}}\right) \]

\end{theorem}

We point that these upper and lower bounds have almost matching dependence on $1-\mu_{i^*}$, differing only in an exponent $M-1$ vs $M+1$.

\begin{proof}

The regret upper bound follows from the same analysis as the gap-independent bound in Agrawal and Goyal. The lemmas we showed establish that the upper bound degrades by at most a constant multiplicative factor and the additive term. We now turn to the lower bound construction.

We make $\mu_1=1-T^{-\frac{1}{M}}$ and $\mu_2=1-2T^{-\frac{1}{M}}$, initialized so $\mu_1\sim Beta(1,M)$ has prior mean $\frac{1}{L+1}$. Suppose that so far $\mu_2$ has been chosen all $t$ times and succeeded each time. Then we have, with $(M,a,b)=(M,t+1,1)$:

\begin{align}\mathbb P[\theta_2(t)\leq\theta_1(t)]&=\binom{M+t+2}{M+1}^{-1}\\
&=O_M(t^{-(M+1)}).\end{align}

Summing over $t$ gives a convergent sum. Hence by Borel-Cantelli, with uniformly positive probability, we will continue to select $a_2$ until its first failure. This has positive probability to happen after time $\Omega(T^{\frac{1}{M}}).$ After this point, a simple martingale argument shows there is a positive chance for $\hat\mu_2(t)$ to stay larger than $1-10T^{-\frac{1}{M}}$ for all times, so that $\theta_2(t)\sim Beta(t+2-b_t,b_t)$ with $b_t\leq 10t\cdot T^{-\frac{1}{M}}$.

For such distributions, conditioned on having no samples of $a_1$, we have 

\begin{align}\mathbb P[\theta_2(t)\leq\theta_1(t)]&= \frac{(M+1)(t+1)!(M+b_t-1)!}{(b_t-1)!(M+t+1)!}\\
&= \Theta_M(b_t^M t^{-M})\\
&= O_M(T^{-1}).\end{align}

Since these probabilities are uniformly summable as $T\to\infty$, we conclude from Borel-Cantelli that with uniformly positive probability, Thompson sampling never plays arm $a_1$. Hence the expected regret is $\Omega(T^{1-1/M})$ as claimed.

\end{proof}



We define a bandit game with \emph{free adversarial exploration} as follows. The player plays a bandit algorithm, and an adversary (with no more information than the player) may adaptively interfere by choosing what arm to play at any time. However, the regret incurred on these rounds is $0$. Certainly the player will not do worse by ignoring the information gathered on these rounds. We argue here that all regret bounds for informative Beta Thompson sampling shown above apply uniformly in the setting of free adversarial exploration.

\begin{theorem}
Suppose we use Thompson sampling with informative Beta prior, but an adversary with the same information as the player can adaptively choose what action to play on some time-steps. However on those timesteps, we receive 0 regret. Then the above upper bounds still apply. 
\end{theorem}

\begin{proof}

The result follows from Lemmas 2.9 through 2.12 in \cite{Shipra-colt12}, so we discuss each of them. Lemma 2.9 is purely an estimate for a beta posterior after a fixed number of samples, so is unaffected (except that some terms will not contribute if the adversary handles those steps, so it actually may help). Lemma 2.10 is generated from Lemma 2.9 and the discussion above it, which is totally unaffected. Lemmas 2.11 and 2.12 again only pertain to a single arm, so the order of exploration is immaterial for them as well. 

\end{proof}

\begin{theorem}

The frequentist regret of our BIC algorithm initialized with an $M$-informative Beta prior satisfies

\[\mathbb E[R(T)]\leq (1+\varepsilon)\sum_{i\neq i^*} \frac{\log(T)}{d(\mu_i,\mu_{i^*})}+O_{\mu}(\varepsilon^{-2})+2^{O_{\mu}(M)}+poly(K,\min(K,M)^M)\]

and \[\mathbb E[R(T)]\leq O\left(\sqrt{KT\log(T)}\right)+O\left(\frac{KM^2\log(T)\mu+KM}{(1-\mu_{i^*})^{M+1}}\right)+poly(K,\min(K,M)^M).\]



\end{theorem}

\begin{proof}

Combine results, paying regret $1$ per timestep during the initial exploration phase.

\end{proof}

==> sec-examples.tex <==
\section{[OBSOLETE] Canonical Examples}
\label{sec:examples}

Here we apply our methods to estimate the exploration complexity $\Tbic{N_{\TS}}$ in some specific cases. For rather general situations we obtain quadratic dependence on $K$. We say that a family $\mathcal C$ of prior distributions $\mu$ is $(c_L,\delta)$-uniformly \emph{BIC explorable} if for any $\mu\in\mathcal C$ we have:

\begin{enumerate}
    \item $\mu^0\geq c_L$.
    \item $\mathbb P[\mu\leq c_L-\delta]\geq \delta$.
\end{enumerate}

This is a natural uniform encapsulation of the requirement that $\mathbb E[(\mu_i^0-\mu_j)_+]>0$ for any arms $i,j$. We now introduce a stronger condition. We say $\mathcal C$ is $(c_L,c_U,\delta)$-uniformly \emph{easily BIC explorable} if it is $(c,L,\delta)$-uniformly BIC explorable and for any $\mu\in\mathcal C$ we have:

\begin{enumerate}
    \item $\mu^0\leq c_U$.
    \item $\mathbb P[\mu\geq c_U+\delta]\geq \delta$.
\end{enumerate}

This condition uniformly encapsulates the condition $\mathbb E[(\mu_i-\mu_j^0)_+]>0$, i.e. that any arm can be better than the prior mean of any other arm. We next show that easily BIC explorable families have sample complexity $O_{c_L,c_U,\delta}(K^2)$ while if not they have (up to edge-cases) sample complexity $e^{\Omega(K)}$. Thus we give an essentially sharp condition for a family $\mathcal C$ of priors to be easy or hard to explore.

\begin{restatable}{theorem}{general}

If $\mathcal C$ is a $\delta$-easily explorable collection of prior distributions, then the exploration complexity satisfies

\[\Tbic{N_{\TS}}=O_{\delta}(K^3).\]

On the other hand, if there exist priors $\mu,\mu'\in\mathcal C$ with $\mu^0= c_U$ and $\mu'<c_U-\varepsilon$ almost surely, then taking $\mu_1,\dots,\mu_{K-1}\sim \mu$ and $\mu_K\sim\mu'$ yields

\[\Tbic{N_{\TS}}\geq e^{\Omega_{c_L,c_U,\varepsilon}(K)}.\]

\end{restatable}

In particular for finite $\mC$ we obtain a precise dichotomy: \mscomment{I think we should name the condition. Maybe when it holds with some $\delta$, $\mC$ is $\delta$-easy (to explore), and if it fails with some $\delta$ margin then $\mC$ is $\delta$-hard (to explore).}

\begin{corollary}

Suppose $|\mC|<\infty.$ If $\min_{\mu\in\mC}\mathbb E[\mu] >\max_{\mu'\in \mC}supp(\mu')$ then $\Tbic{N_{\TS}}=e^{\Omega_{\mC}(K)}$ while if $\min_{\mu\sim \mC}\mu_0^1 <\max_{\mu'\sim \mC}supp(\mu')$ then $\Tbic{N_{\TS}}=O_{\mC}(K^2).$

\end{corollary}

We now turn to two canonical examples: Gaussians (truncated to lie in $[0,1]$) and beta priors. We investigate the dependence of $\Tbic{N_{\TS}}$ on the parameters of the Gaussian and beta priors.

\begin{restatable}{theorem}{gaussianbound-old}
Let $\tilde N(m,\sigma^2)$ be a Gaussian with mean $m$ and variance $\sigma^2$, conditioned to lie in $[0,1]$. Suppose $\mu_i\sim \tilde N(m_i,\sigma^2)$ for each arm $i$, where
    $m_1 \LDOTS m_K\in [0,1]$.
Then the exploration complexity is $\Tbic{N_{\TS}} = \poly(K,\sigma^{-1},e^{R^2})$,
where
    $R=\sigma^{-1}\;\max_{i,j} |m_i-m_j|$.
\end{restatable}

\vspace{-3mm}

\begin{restatable}{theorem}{betabound-old}
Let $\mu_i\sim \term{Beta}(a_i,b_i)$ for each arm $i$, where $a_i,b_i\leq M$. Then the exploration complexity is
$\Tbic{N_{\TS}} \leq K^3\cdot \rbr{O(\min(K,M))}^{O(M)}$.
%$\Tbic{N_{\TS}} \leq K^2\cdot M^{O(M)}$. \msedit{Moreover this is achievable by a $poly(K,M)$-per-time-step algorithm.}
\end{restatable}

\begin{remark}\label{rem:deep-reason}
Fixing the prior mean rewards, the exploration complexity in these two examples is driven by the parameters $\sigma^{-1}$ and $M$, respectively, and is increasing in these parameters. Each parameter  characterizes the strength of beliefs in the corresponding example.
\end{remark}


\msedit{In the next result we show that when the top action is highly informed while the others are uninformed, the exploration complexity is small. This is a natural situation to study because blahblahblahpleasefillin}

\begin{restatable}{theorem}{realistic}
Suppose $\mu_1\sim \term{Beta}(a_1,b_1)$ for $a_1,b_1\leq M$ while $\mu_i\sim \term{Beta}(a_i,b_i)$ for $a_i,b_i\leq m$. Then

\[\Tbic{N_{\TS}} \leq  MK^2\cdot \max(m,(1-\mu_1^0)^{-1})^{O(m)}.\]


\end{restatable}








%one can  you can assume there is one bad arm and the rest iid good arms.
%And then you compute the parameters epsndg, nexplore, L in thm 22.
%Using q uniform over the K-1 good arms which you can assume by symmetry



==> sec-junk.tex <==
\section{JUNK to make things compile / for compatibility}

% \begin{restatable}{lemma}{easyexploreparameters}
% \label{lem:easyexploreparameters}
% If $\mC$ is $\delta$-easy to explore, then:
% \begin{itemize}
%     \item $N_{\TS}=\tilde O(K\delta^{-2})$.
%     \item $G\geq \delta$.
%     \item $\padN=\tilde O(\delta^{-2}).$
%     \item $\bootN=\tilde O(\delta^{-1})$.
%     \item $\log(\Pexplore^{-1})=\tilde O(K\delta^{-1})$.
% \end{itemize}
% \end{restatable}


%\begin{restatable}{lemma}{easybound}
%\label{lem:easybound}
%Suppose some BIC algorithm explores each arm almost surely in $T_0$ rounds. Then
%    $T_0\geq \max(K,N_{explore},L)$,
%where
%\[L=\max_{j\in [K],q\in \Delta_{K}}\frac{\mathbb E[(\mu_j-\mu_q)_-]}{\mathbb E[(\mu_j-\mu_q)_+]}=\max_{j\in [K],q\in \Delta_{K}}\frac{\mu_q^0-\mu_j^0}{\mathbb E[(\mu_j-\mu_q)_+]}-1.\]
%\end{restatable}
%
%
%\begin{restatable}{theorem}{tscomplexity}
%\label{thm:tscomplexity}
%Assume the priors are $\EpsNdg$-non-degenerate. Then Algorithm~\ref{alg:pyramidtight} achieves $N_{\TS}$ samples of each arm within
%\[\Tbic{N_{\TS}} =\tilde O\left(\frac{K^{9/2}L^3\Nexplore}{\EpsNdg^4}+\frac{K^{5/2} L\Nexplore^2}{\EpsNdg^{2}}\right)\]
%
%timesteps. Moreover a faster version, Algorithm~\ref{alg:pyramidtightfast}, achieves $N_{\TS}$ samples of each arm within
%
%\[\Tbic{N_{\TS}}= O\left(\frac{K^{7/2}L^3\Nexplore}{\EpsNdg^4}\right).\]
%time steps.
%
%\end{restatable}
%
%\begin{remark}\label{rem:alg2}
%We also provide a more elaborate algorithm (see Algorithm~\ref{alg:pyramidtightfast} in Appendix~\ref{}) which collects $N$ samples of each arm almost surely in time
%\begin{align}\label{eq:better-algo}
% \RndsUBtwo(N) = O\rbr{ K\;\padG^{-1}\;
%    \rbr{N + \bootN + \padN\, \log\rbr{\bootP^{-1}}}}.
% \end{align}
%This shaves off a factor of $\log\rbr{\bootP^{-1}}$ from $\RndsUB(N)$
%    when $N\gg \padN$,
%and leads to tangible improvements in some examples in Section~\ref{sec:examples}. The idea is to implement \MainALG using phases of $\padN$ rounds each, and obtain the remaining $N-\padN$ samples in the very end.
%\end{remark}
%
%The algorithm from Remark~\ref{rem:alg2} achieves a somewhat better bound compared to \eqref{eq:thm:matching}:
%\begin{align}\label{eq:thm:matching-two}
%\RndsUBtwo(N_{\TS})
%    \leq \tildeO\rbr{ \sigma^{-4}\, K^{3.5}\, \MainLB^3\,\bootN}
%\end{align}
%under the assumptions in Theorems~\ref{eq:thm:matching} and~\ref{eq:thm:matching-improved}, which helps \ascomment{where?}.
%
%
%In fact, the algorithm from Remark~\ref{rem:alg2} achieves
%    $\RndsUBtwo(N_\TS)= O_\mC(K)$
%under the same condition, which is the optimal dependence on $K$ even without the BIC constraints.
%
%\mscomment{The second algorithm only achieves $O_{\mC}(K^2)$. There is a third algorithm I haven't written up yet which gets $O_{\mC}(KN_\TS)$ by picking a random arm at the start and only ever exploiting that one (crazy right??? There are still a bunch of other parameters like $N_{pad}$ but they are $O(1)$ for fixed $\mC$). In the worst case (as far as I can prove) $N_{\TS}=\Omega(K)$ might be possible, but this at least gives $\tilde O_{\mC}(K)$ for beta priors.}
%



==> sec-prelims-partial.tex <==
\subsection{Partial strategies and their BIC properties}

%\xhdr{Versions of the BIC property.}

% We define various weaker versions of the BIC property using the identity
% \[\E[\mu_k\mid A_t=a_k,\, \mE_{t-1}]
%     =\frac{\E[\mu_k\cdot 1_{A_t=a_k}]}{\mathbb P[A_t=a_k,\, \mE_{t-1}]}.\]

\begin{definition}
Fix round $t$ and condition on the event $\mE_{t-1}$.
An algorithm is \emph{BIC at time $t$} if
    \[\E[\mu_k \mid A_t=a_k,\mE_{t-1}]\geq \E[\mu_j \mid A_t=a_k]\]
holds for all arms $k,j$, or equivalently if
\begin{align}\label{eq:BIC-defn-2}
    \E[\mu_k\cdot 1_{A_t=a_k}]\geq \E[\mu_j\cdot 1_{A_t=a_k}].
\end{align}
(Note that the algorithm is BIC if it is BIC for all rounds $t$.)
If \eqref{eq:BIC-defn-2} holds for a specific arm $k$ and all arms $j$, then we say the algorithm is \emph{$k$-BIC at time $t$}. If \eqref{eq:BIC-defn-2} holds holds for a specific $(k,j)$ pair we say the algorithm is \emph{$k$-BIC for arm $j$ at time $t$}.
\end{definition}

We use \emph{strategy} to refer to an algorithm's behavior at a fixed time $t$. Formally, it is a (possibly randomized) mapping from the observed history to actions.
We define a \emph{partial strategy} at time $t$ to be a strategy which is defined only for some $\mF_t$-measurable subset of events.%
\footnote{More pedantically, it is a pair consisting of a $\mF_t$-measurable subset and a strategy on that subset.} For instance, restricting a strategy at time $t>1$ to the event that $a_1$ earns reward in round $1$ yields a partial strategy. We similarly say a partial strategy is BIC if it satisfies \eqref{eq:BIC-defn-2} for all arms $(k,j)$, and that it is $k$-BIC if the inequality is satisfied for a fixed arm $k$ and all arms $j$. We say a strategy is \emph{full} to emphasize that it is well-defined with probability $1$.

% By linearity, any mixture or union of BIC partial strategies is BIC.

We define a partial strategy that is BIC \emph{and} moreover it is $k$-BIC with some margin:
\begin{definition}
A partial strategy is called $(k,\alpha)$-BIC at time $t$, for arm $k$ and $\alpha\geq 0$, if it is BIC and moreover for all arms $j\neq k$ it holds that
\[\E[(\mu_k - \mu_j)\cdot 1_{A_t=k}| \mE_{t-1}]\geq \alpha.
\]
\end{definition}

Let us present several basic lemmas on how to combine these concepts. First, we note that the $(k,\alpha)$-BIC property of a partial strategy $\mS$ is preserved if $\mS$ is completed by playing \emph{greedily}, \ie choosing an arm that maximizes posterior mean reward given the current observations.

\begin{proposition}\label{prop:kBICextend}
Any $(k,\alpha)$-BIC partial strategy extends to a $(k,\alpha)$-BIC strategy by playing ``greedily" on the ``undefined event" (the set of outcomes for which the partial strategy is not defined).
\end{proposition}

Second, we encapsulate the ``hidden exploration" technique from \citet{ICexploration-ec15}. The formulation below follows, \eg from Lemma 11.13 in \citet{slivkins-MABbook} and means that $(k,\alpha)$-BIC partial strategies give some breathing room.

\begin{lemma}\label{lem:replaceaction}
Suppose $\mS$ is a partial strategy which is $(k,\alpha)$-BIC at time $t$. Suppose that at time $t$, with probability $\frac{\alpha}{2}$ we play action $k$ and with probability $1-\frac{\alpha}{2}$ we play using $\mS$. This modified strategy is BIC at time $t$.
\end{lemma}

Third, we combine partial policies defined on disjoint events.

\begin{proposition}\label{prop:BICmixture}
Suppose the algorithm plays arm $k$ at time $t$ exactly on the disjoint union of two $\mF_t$-measurable events $E_1,E_2$, and that playing arm $k$ on each event separately is BIC for $k$. Then the algorithm is also BIC for arm $k$ at time $t$.
\end{proposition}

\begin{proof}
Simply observe that $\E[\mu_j\cdot 1_{A_t=a_k}]=\E[\mu_j\cdot 1_{E_1}]+\E[\mu_j\cdot 1_{E_2}]$ for all $j$.
\end{proof}



==> sec-pyramid-2020-01-19.tex <==
\section{[OLD/OBSOLETE] How Many Rounds Does It Take to Sample Every Arm?}
%\label{sec:sampling}

%Initial Sampling via the Pyramid Scheme
%\label{sec:algorithm}

We revisit the basic sample complexity question for incentivized exploration: how many rounds does it take to obtain $N$ samples from each arm? This is the waiting time before switching to Thompson sampling, as per Theorem~\ref{thm:TSsamples}, if  $N=N_{\TS}$.

We design a BIC algorithm \MainALG, whose performance guarantee is stated as follows.

%we now seek to efficiently acquire samples of each arm. We ask for a BIC algorithm which by a fixed time $T$ always achieves at least $\Nsamples$ samples of each arm, and seek to minimize $T$. For $\Nsamples\geq N_{\TS}$, this is the amount of waiting time before Thompson sampling can be implemented.


% \begin{restatable}{theorem}{goodalgo}
% \label{thm:goodalgo}
% Algorithm \MainALG is BIC. Given parameter
%     $\Nsamples\geq \max(N_{\post},\Nexplore)$,
% it obtains $\Nsamples$
% samples of each arm almost surely in time
% \[ \Tbic{N} = O\paren{
%     KN\;G^{-1} \log(\Pexplore^{-1})
% }.\]

% \end{restatable}

% Under the assumption that $\Pr[\mu_j<1-\eps_0]>\delta_0$ for all $j$ we obtain the mild $(\eps_0,\delta_0)$ dependence $O\left(\frac{K\Nsamples(K\eps_0^{-1}+\log(\delta_0^{-1}))}{\eps_{\post}\delta_{\post}}\right)$

%\[O\left(K\left(\Nsamples+\eps_{\post}\delta_{\post}\log\left(\frac{1}{\Pr[E_k]}\right)\right)\right).\]

%\[O\left(K\left(\Nexplore+\frac{1}{\eps_{\post}\delta_{\post}}\left(N_{\post}\log\left(\frac{1}{\Pr[E_k]}\right)+N_{\TS}\right)\right)\right).\]


\begin{definition}\label{def:params}
Let us define the prior-dependent parameters $N_{\post}, \Nexplore, G,\Pexplore$.

First, let $E_{i,L}$ be the event that the first $L$ samples of each arm $j<i$ return reward $0$. Let
\begin{align}\label{eq:-defn-Nexplore}
\Nexplore = \min \left\{ L\in\N:\;
    \E[ \mu_i-\mu_j \mid E_{i,L}] > 0
    \qquad \text{for all arms $i>j$}
\right\}.
\end{align}
In words, this is the smallest $L$ such that each arm $i$ is the best arm conditional on event $E_{i,L}$.
\begin{align}\label{eq:-defn-Pexplore}
\Pexplore = \min_{\text{arms $i$}} \Pr[E_i],
\quad\text{where}\quad E_i := E_{i,\;\Nexplore}.
\end{align}

Second, letting $\mu_q = \E_{i\sim q}[\mu_i]$ for distribution $q$ over arms,
\begin{align}\label{eq:defn-G}
G=\min_{i\in [K],\;q\in \Delta_{i-1}}\E\left[\left(\mu_i-\mu_q\right)_+\right].
\end{align}
In words, this is the smallest ``expected advantage" of any arm $i$ over a convex combination of arms $j<i$. Finally, let
\begin{align}\label{eq:defn-Npost}
 N_{\post} = \Theta(G^{-2} \log (G^{-1}) )
 \quad\EqComment{with large enough constant in $\Theta()$}.
\end{align}
\end{definition}

\begin{remark}
The meaning of this result is three-fold. First, it is an explicit formula for the sample complexity in question, even if it invokes several prior-dependent parameters. Second, this formula is polynomially optimal, see Section~\ref{sec:LB}. Third, this formula is \emph{productive} for some paradigmatic special cases, see Section~\ref{sec:LB}: we obtain a polynomial dependence on the number of arms.
\end{remark}

\subsection{Our algorithm}

Call a given arm \emph{explored} if it has been sampled at least $\Nsamples$ times. \mscomment{I'm thinking $N$-explored is probably clearer, right?} %For the sake of intuition, let us assume that
%the arm's mean reward is known exactly when this happens.
We explore the arms in order of increasing index (\ie in the order of decreasing the prior mean reward). Having explored arms $1 \LDOTS j-1$, we explore arm $j$ as follows. We partition time in phases of $\Nsamples$ rounds each. Within a given phase, we recommend the same arm in all rounds. There are three options:

\begin{itemize}
\item[(i)] we \emph{explore} by recommending arm $j$,
\item[(ii)] we \emph{exploit} by recommending an arm with the largest posterior mean reward,
\item[(iii)] we \emph{exploit-with-bias} by recommending an arm according to a $(j,G/10)$-BIC strategy.
\end{itemize}

In the first phase, we \emph{explore} if event $E_j$ has happened, and \emph{exploit} otherwise. In each subsequent phase $\ell$, we have two cases, depending on whether arm $j$ has already been explored. If it hasn't, then we \emph{explore} with small but exponentially growing probability, and exploit otherwise. If arm $j$ has already been explored, then we \emph{exploit-with-bias}. We iterate this loop while the exploration probability is less than $1$. The pseudocode can be found in Algorithm~\ref{alg:pyramidtight}.

Compared to the \emph{hidden exploration} technique from prior work (\citet{ICexploration-ec15}, see Ch. 11.4 in \citet{slivkins-MABbook} for exposition), we have two key innovations: an exponentially growing exploration probability and the \emph{exploit-with-bias} option. Growing the exploration probability is possible because the more likely we are to have already explored arm $j$, the more likely it becomes that the exploitation choice is arm $j$, too. Exploration has a compounding effect, as each exploratory phase gives the planner more leverage to explore arm $j$ in future rounds.


%While exploration is wasted whenever arm $j$ is not the best arm, a small fraction of explorations bear lasting fruit. The successful explorations


\begin{figure}[t]

\SetKwFor{Loop}{loop}{}{end}

\begin{algorithm2e}[H]%\label{alg:pyramidtight}
%\caption{\MainALG}

\SetAlgoLined\DontPrintSemicolon

\textbf{input:} $N$, the desired number of samples;
parameters from Definition~\ref{def:params}.

\For{$j=1,2,\dots,K$}{ \label{line:algloop}
\tcp*[f]{Obtain $N$ samples of arm $j$ a.s.}

Set $p_j=\Pr[E_j]$.\\

\uIf{$E_j$}{
Choose arm $j$ for the next $N$ rounds.
\tcp*[f]{explore}
}

\uElse{
Exploit for the next $N$ rounds.

}

\tcp*[f]{Now we grow the exploration probability}

Compute strategy $S_j$ which is $j$-correlated and
    $\left(j,\frac{G}{10},[j-1]\right)$-BIC for $\mathcal G_{N,j}$ coming from Lemma~\ref{lem:BICmargin}.
\tcp*[f]{exists by Lemma~\ref{lem:BICmargin}. }


\While{$p_j\leq 1$}{
\uIf{arm $j$ has been explored already}{
Use $S_j$ for the next $N$ rounds
\tcp*[f]{exploit-with-bias}
}
\uElse{
With probability $\frac{p_j}{1-p_j}\cdot \frac{G}{10}$, play arm $j$ for the next $N$ rounds; \label{line:algexplore}
\tcp*[f]{explore}

\tcp*[f]{arm $j$ is now explored with probability $p_j$}

with the remaining probability, exploit for the next $N$ rounds.
%Play the arm with highest $\mathcal F_t$-posterior mean for the next $N$ rounds.
}
$p_j\leftarrow p_j\cdot \left(1+\frac{G}{10}\right)$
}%end while
} %end for
\end{algorithm2e}
\end{figure}

The number of rounds is as claimed in Theorem~\ref{thm:goodalgo} because there are
    $O\left(G^{-1}\log (\Pexplore^{-1}) \right)$
phases for each of the $K$ arms, each of which lasts for $N$ rounds.

\begin{remark}
The algorithm is not computationally efficient, because it needs to compute strategy $S_j$ for each arm $j$ (which is a very large object: an entire mapping from histories to actions). It can be done by solving a large zero-sum game up to high precision, which is feasible but slow. \mscomment{I think in the Gaussian and Beta examples there will be an efficient version of the algorithm with similar performance, not sure where to describe it.}
\end{remark}

\begin{remark}
In the Appendix we also give a version of \MainALG (Algorithm~\ref{alg:pyramidtightfast}) with a somewhat smaller number of rounds for large $N$. The idea is to implement \MainALG using phases of $N_{\post}$ rounds, and obtain the remaining $N-N_{\post}$ samples in the very end.
\end{remark}
%The reason that it is BIC is essentially Lemma~\ref{lem:replaceaction}

\subsection{Proof Sketch: the algorithm is well-defined}

To make the algorithm well-defined, we need to prove that the  $\left(j,\frac{G}{10}\right)$-BIC strategy $S_j$ exists. This follows from the two lemmas below. The first lemma is a consequence of the Bayesian Chernoff bound (Lemma~\ref{lem:TSchernoff}).

%To make the outline in the previous subsection precise, we must estimate the number of samples required for myopic exploration to significantly exploit a given arm $a_j$. This will give us leverage to explore $a_j$ when it has not been explored.



% \begin{restatable}{lemma}{chernofftwo}
% \label{lem:chernoff2}
% Fix arm $k$ and time $T_0$. Suppose for some $q\in\Delta_{k-1}$ and
%     $\eps_{\post},\delta_{\post}>0$,
% \[ \Pr\left[\left(\mu_k-\mu_q\right)_+ \geq \eps_{\post}\right]\geq \delta_{\post}.\]
% Let \ALG be a BIC algorithm which by time $T_0$ collects at least $N_{\post}$ samples of each arm $j\in [k]$ a.s., where
% \[N_{\post}\geq
% 100\;\eps_{\post}^{-2}
% \left(1+\log\left(\eps_{\post}^{-1}\cdot\delta_{\post}^{-1}\right)
% \right)\]
% Let $\mathcal G_{N_{\post},k}$ be the $\sigma$-algebra generated by the first $N_{\post}$ samples of each of these $k$ arms. Then
% \[\E\left[\left(\E\left[\mu_k-\mu_q \mid \mathcal G_{N_{\post},k}\right]\right)_+\right]\geq \frac{\E[(\mu_k-\mu_q)_+]-\delta_{\post}-\eps_{\post}}{2}.\]

% \end{restatable}

This feeds into the next Lemma, which shows how to turn exploration back into exploitation. The proof relies crucially on both the minimax theorem and the FKG inequality (see Appendix~\ref{app:mon-ineq}).

% \begin{restatable}{lemma}{BICmargin}
% \label{lem:BICmargin}
% Fix arm $k$ and $\alpha>0$. Suppose there exists a static $\sigma$-algebra $\mathcal G_k=\mathcal G_{N_1,N_2,\dots,N_k,0,\dots,0}$ which is independent of
%     $(\mu_{k+1}  \LDOTS \mu_K)$
% and satisfies
% \[\E\left[\left(\E\left[\mu_k-\mu_q\mid \mathcal G_{k}\right]\right)_+\right]
% \geq \alpha \quad\text{ for all }q\in\Delta_{k-1}.\]
% Then there exists a $\mathcal G_k$-measurable $(k,\alpha,[k-1])$-BIC strategy for the planner. \msedit{Moreover, this strategy only plays arms in $[k]$, and satisfies \[\mathbb E[\mu_i|A_t=i]\geq \mu_i^0,\quad \mathbb E[\mu_i|A_t=j]\leq \mu_i^0\] for any $i\leq k,j\leq k$ with $i\neq j$.}

% \mscomment{$(k,\alpha,[k-1])$-BIC is supposed to mean it is $\alpha$-BIC against arms $[k-1]$ and $0$-BIC against the later ones.}

% \end{restatable}

\msedit{We remark that if the values $(\mu_i\colon i<k)$ are known exactly then a $(k,G)$-BIC strategy exists, and $G$ is the largest value for which this is true. The idea of the proof is to construct a two-player zero-sum game in which a planner recommends some arm $P\leq k$ and then the agent plays an arm $A\leq k-1$, and the planner's payoff is $(\mu_P-\mu_A)\cdot 1_{P=k}$. Letting the agent move first shows that $G$ is exactly the minimax value of the game, while letting the planner go first then shows that a $(k,G)$-BIC strategy exists. The purpose of Lemmas~\ref{lem:chernoff2},~\ref{lem:BICmargin} is to estimate the number of samples needed to ensure the (average) value of this game is at least $G/10$.}

\begin{remark}
Lemma~\ref{lem:BICmargin} motivates the definition of parameter $G$ in \eqref{eq:defn-Npost}. We fix
    $\eps_{\post},\delta_{\post}=\frac{G}{10}$.
Then the assumption (and hence conclusion) of Lemma~\ref{lem:chernoff2} holds for all $k\in [K]$ and $q\in \Delta_{k-1}$. In particular the two descriptions of $N_{\post}$ are seen to agree.
\footnote{In general, if $X\in [0,1]$ is a random variable with $\E[X]\geq \alpha$ then $\mathbb P[X\geq \alpha/10]\geq \alpha/10$.}
\end{remark}

\msedit{The idea of the algorithm is that a $(k,G/10,[k-1])$-BIC strategy in the event that $a_k$ is already explored allows us to grow the exploration probability by a factor of $\left(1+\frac{G}{10}\right)$ each iteration. The $G/10$ margin in the BIC condition unlocks some additional exploration proportional to the exploration probability accumulated so far. There are some technical points that must be addressed to ensure the algorithm is BIC. For example, the event that $a_k$ is explored is not independent of the values $(\mu_i)_{i\leq k-1}$, which could conceivably prevent a $(k,G/10,[k-1])$-BIC strategy from existing. Moreover we must ensure that Algorithm~\ref{alg:pyramidtight} is also BIC against arm $a_{k+1}$. These properties are shown to hold throughout via careful application of the FKG inequality.}


\subsection{Outline of the Algorithm in a Special Case}

Focus on a lucid special case, where we improve the number of rounds to $\poly(K)$ (as compared to $\exp(K)$ in prior work). We suppose arm $K$ -- the one with the lowest prior mean reward -- satisfies $\mu_K \sim \term{Beta}(1,2)$, call it the ``bad arm". Whereas $\mu_i$ is distributed uniformly on $[0,1]$ for all other arms $i<K$, call them ``good arms".

Let $\Lambda = \frac{1}{K-1}\;\sum_{j=1}^{K-1} \mu_j$ be the average true mean reward of the good arms. Observe that with probability
    $1-\Pr\left[\mu_K^0>\Lambda\right]$,
which is exponentially close to $0$, the average of the $K-1$ good arms is well above $\mu_K^0=\frac{1}{3}$. Therefore, it seems very difficult to obtain initial samples of arm $K$: the agent would have to assign enough credence to this exponentially unlikely event to prefer $a_K$ to a uniformly random good arm. However, if we only wish to explore $a_K$ on this exponentially unlikely event, we may certainly do so in a BIC manner because the $K-1$ good arms are symmetric. In this way, after $O(K)$ rounds to obtain $O(1)$ initial samples of each good arm, we have probability $e^{-\Theta(K)}$ to be able to explore arm $K$. Now conditioned on having explored $a_K$ (and ignoring the confounding that we explore arm $K$  when the good arms are unusually bad, which only helps), we have an expected $\E\left[\left(\mu_K-\Lambda\right)_+\right]=\Omega(1)$
amount of potential exploitation per future round by playing $a_K$. This is because the true value $\mu_K$ of $a_K$ has a very reasonable $\Omega(1)$ chance to be at least $0.8$ (say). More generally, if at some point we have explored $a_K$ with probability $p_t$, then we may leverage exploitation in those cases to play an unexplored $a_K$ with probability $\Omega\left(p_t\right)$ for the next $\Nsamples$ rounds. Roughly, in timestep $t$ the algorithm will have explored $a_K$ with probability
    \[\Pr\left[\mu_K^0>\Lambda\right]\cdot \left(1+\E\left[\left(\mu_K-\Lambda\right)_+\right]\right)^{t/\Nsamples}.\]
Due to the exponential growth of the exploration probability, this expression reaches $1$ quickly and the bad arm can be explored in $\poly(K)$ time.

%To speed things up in the final algorithm, we only carry out the exponential growth using a smaller number $N_{\post}$ of samples per arm, and then obtain the full required number of samples at the end.




% \subsection{Efficiently Computable Algorithm}

% So far we gave an algorithm and showed its sample efficiency is optimal up to polynomial dependency. However computing it requires solving an exponentially large two player zero sum game to high precision and hence does not seem tractable in full generality. Here we give a variant which is efficiently computable and is sample efficient in many examples. However, there are examples where it is exponentially inefficient. The idea is to only exploit $a_k$ when $\mu_k$ has the highest posterior mean. We require two additional parameters $\eps_{pre},\delta_{pre}$ such that

% \[\Pr[(\mu_k^0-\mu_j)_+>\eps_{pre}]\geq \delta_{pre}\]

% for all $k,j$. Define \[N_{pre}=\left(\frac{1000\left(1+\log\left(\frac{1}{\eps_{pre}\cdot\delta_{pre}}\right)\right)}{\eps_{pre}^2}\right).\]



% \ms{Fix statement of Theorem}

% \begin{restatable}{theorem}{efficientpyramid}

% \label{thm:efficientpyramid}

% For any $\Nsamples\geq \max(N_{\TS},N_{pre},N_{\post})$, there is an efficient BIC algorithm which obtains $\Nsamples$ of each arm almost surely in $O\left(\frac{K\cdot \Nsamples\cdot\log(\delta_{pre}^{-1})}{\eps_{pre}\eps_{\post}\delta_{\post}}\right)$ time steps.

% \end{restatable}


==> sec-pyramid-2021-02-04.tex <==
\section{Collecting Initial Samples}
\label{sec:sampling}

We turn to a basic version of incentivized exploration: collect $N$ samples of each arm. We design a BIC algorithm, called \MainALG, which completes after a pre-determined number of rounds and collects $N$ samples of each arm almost surely.
(This is a desirable property as per Remark~\ref{rem:switch-time}.)
We bound the completion time in terms some parameters of the prior.


%how many rounds does it take to obtain $N$ samples from each arm almost surely? This is the ``waiting time" before switching to Thompson Sampling, as per Theorem~\ref{thm:TSsamples}, if  $N=N_{\TS}$.


%we now seek to efficiently acquire samples of each arm. We ask for a BIC algorithm which by a fixed time $T$ always achieves at least $\Nsamples$ samples of each arm, and seek to minimize $T$. For $\Nsamples\geq N_{\TS}$, this is the amount of waiting time before Thompson sampling can be implemented.


%Call a given arm \emph{explored} if it has been sampled at least $\Nsamples$ times.

We describe the algorithm on a high level, and then fill in the details.
We explore the arms in order of increasing index, \ie decreasing prior mean reward. A given arm $j$ is explored as follows. We partition time in phases of $N$ rounds each. Within a given phase, we recommend the same arm in all rounds. There are three options: ``pure exploration", when we always recommend arm $j$, ``pure exploitation", when we choose an arm with the largest posterior mean reward and recommend this arm throughout the phase, and a ``padded phase" which combines exploration and exploitation and enables an exponential boost in efficiency. In the ``padded phase", arm $j$ is recommended sufficiently often and for a sufficiently good reason so as to guarantee a stronger BIC property for arm $j$. This property is parameterized by a prior-dependent amount $\padding >0$. We think of this amount as ``padding", and leverage it to offset additional ``pure exploration".

%We guarantee that the ``pure exploration" phase is invoked almost surely

Algorithm~\ref{alg:pyramidtight} presents the algorithm with abstract parameters $N_0\leq N$ and $\padding>0$, and recommendation policies for the padded phase. Let us again focus on exploring a particular arm $j$. The three phases described above are interleaved in a somewhat intricate way. For bootstrapping, we have one phase in which we explore if the first $N_0$ samples of all previous arms $i<j$ returned zero rewards, and exploit otherwise. Then, we enter a \term{while} loop, where we grow the \emph{phase-exploration probability}: the probability that the ``pure exploration" phase for arm $j$ has been invoked. Once this happens, we permanently switch to the ``padded phase". Meanwhile, we randomize between ``pure exploitation" and ``pure exploitation" with predetermined probability. The latter is chosen to ensure that the phase-exploration probability is boosted by the factor $1+\padding$ at each iteration. This process continues until the phase-exploration probability reaches $1$.


\begin{figure}[t]
\SetKwFor{Loop}{loop}{}{end}

\begin{algorithm2e}[H]\label{alg:pyramidtight}
\caption{\MainALG}
\SetAlgoLined\DontPrintSemicolon

\textbf{Parameters:}
    phase length $N$,
    bootstrapping parameter $N_0\leq N$,
    padding $\padding>0$.

\textbf{Given:}
recommendation policies $\pi_2 \LDOTS \pi_K$ for \PaddedPhase.

\asedit{\ExplorePhase[1].}

\For{each arm $j=\asedit{2}  \LDOTS K$}{ \label{line:algloop}
    \tcp*[l]{Invariant 1: each arm $i<j$ has been sampled $\geq N$ times.}

    \tcp*[f]{the bootstrapping phase}

    Set $\ZEROS_{j,N_0} = \{\text{the first $N_0$ samples of each arm $i<j$ return reward $0$}\}$

    \uIf{$\ZEROS_{j,N_0}$}{\ExplorePhase}
        \uElse{\ExploitPhase.}



    \tcp*[f]{grow the exploration probability}\\
    Set $p_j=\Pr\sbr{\ZEROS_{j,N_0}}$.

    \While{$p_j< 1$}{
    \tcp*[l]{Invariant 2: $\Pr\sbr{\text{exploration phase has happened}}=p_j$}
    \uIf{exploration phase has happened}{
        \PaddedPhase: use policy $\pi_j$ for the next $N$ rounds
        }
    \uElse{
    With probability $\min\rbr{1,\,\frac{p_j}{1-p_j}\cdot \padding}$, \ExplorePhase; \label{line:algexplore}
    \\with the remaining probability: \ExploitPhase.
}
$p_j\leftarrow \min\rbr{1,\, p_j\, (1+\padding)}$
}%end while
} %end for
\end{algorithm2e}
\end{figure}

Let's make some observations that are immediate from the algorithm's specification.

\begin{claim}\label{cl:alg-obs}
The algorithm completes in
    $N+N\,\sum_{j=2}^K \ln_{1+\padding} \rbr{1/\Pr[\ZEROS_{j,N_0}]}$
rounds, and samples each arm at least $N$ times almost surely. \asedit{Both invariants hold.} The bootstrapping phase is BIC as long as
\begin{align}\label{eq:cl:alg-obs:boot}
 \E\sbr{ \mu_j-\mu_i \mid \ZEROS_{j,N_0} } \geq 0
    \quad \text{for all arms $i<j$}.
\end{align}
\end{claim}

The key is to specify what happens in the ``padded phase", and argue about  incentives that it creates.
The recommendation policy $\pi_j$ for a given arm $j$ needs to satisfy several properties in addition to being BIC.
\begin{itemize}

\item First and foremost, we require a stronger BIC property for arm $j$:
\begin{align}\label{eq:padded-BIC-defn}
\E\sbr{ (\mu_j - \mu_i)\cdot \ind{\pi_j=j}}\geq \padding
\quad\text{for each arm $i<j$}.
\end{align}
We say that policy $\pi_j$ is \emph{$(j,\padding)$-padded BIC} if \eqref{eq:padded-BIC-defn} holds, where $\lambda$ is the ``padding".
The left-hand side in \eqref{eq:padded-BIC-defn} is the expected loss for the $j\to i$ swap: the expected loss when one starts with policy $\pi_j$ and replaces arm $j$ with arm $i$ whenever arm $j$ is recommended. Note that we integrate over the event that arm $j$ being chosen, rather than condition on this event.

\item Second, we require $\pi_j$ to input only the first $N$ samples of each arm $i<j$; such policies are called $(j,N)$-informed. This property ensures that the algorithm has sufficient data to compute policy $\pi_j$.


\item Third, we focus on the probability of recommending arm $j$ as a function of the posterior mean rewards
    $\widetilde{\mu}_i := \E\sbr{ \mu_i \mid \mathcal \mG_{N,j}}$,
    for each arm $i\leq j$.%
    \footnote{Recall that $\mG_{N,j}$ denotes the $\sigma$-algebra generated by the first $N$ samples of each arm $i\leq j$.}
    We posit that the conditional probability
        $\Pr\sbr{ \pi_j = j \mid \widetilde{\mu}_1 \LDOTS \widetilde{\mu}_j }$
    is monotonically  non-decreasing in $\widetilde{\mu}_j$ and monotonically non-increasing in $\widetilde{\mu}_i$ for each arm $i<j$. Such $\pi_j$ is callled \emph{$j$-correlated} given $\mG_{N,j}$.
    This is a natural property for a BIC recommendation policy that strives to explore arm $j$. We use it to apply the FKG inequality.

\end{itemize}
If policy $\pi_j$ is BIC and satisfies all three properties, it is called \emph{$(j,\padding,N)$-suitable}.


\asedit{We show that these properties guarantee the \term{while} loop to be BIC. The main point is that the $(j,\lambda)$-padded property of policy $\pi_j$ compensates for the probability of new exploration.  The exploitation phase is only used to skip the round in a BIC way.%
\footnote{\asedit{This is an interesting contrast with ``hidden exploration" \citep{ICexploration-ec15}, where the exploitation phase is used to offset exploration. We have little use for this, because the padded phase enables nearly as much additional exploration as possible.}}
We rely on the FKG inequality to handle various technicalities.}

%A technical point is that being in the padded phase is not independent of the values $(\mu_i)_{i\leq j})$ due to the use of events $\ZEROS_{j,N_0}$ to start the exponential growth. Additionally, we must show that the BIC property continues to hold against the future arms $a_i$ for $i>j$. We handle both points by using the FKG inequality.

%We remark that our padded phase has the same functionality that the exploitation phase does in \cite{ICexploration-ec15}. By contrast, our exploitation phase is only used to skip the round in a BIC way. This is because by construction, our padded phase accounts for essentially as much additional exploration as possible, so in a sense all the value has been extracted out of the exploitation phase.


\begin{lemma}\label{lm:main-BIC}
Consider algorithm \MainALG with arbitrary parameters $N_0\leq N$ and $\padding>0$.
Fix some arm $j\geq 2$. The $j$-th iteration of the \term{while} loop is BIC as long as policy $\pi_j$ is $(j,\padding,N)$-suitable.
\end{lemma}

\renewcommand{\IndPadded}{\indE{\term{padded}}}
\renewcommand{\IndExplore}{\indE{\term{explore}}}
\renewcommand{\IndExploit}{\indE{\term{exploit}}}

\renewcommand{\padExpr}{\Lambda^{\term{pad}}_{i,j}}

\begin{proof}
% \mscomment{The proof still has to use FKG a few times, so I think a proof outline may be better.}
% The main point is that if we use $\pi_j$ with probability $p_t$ on round $t$, then this ``by definition" cancels out the non-BICness of $\lambda p_t$ probability of exploration. The stipulation of being $j$-correlated allows us to use the FKG inequality to verify, for instance, that the fact that the initial exploitation phase was dependent on the previous arms only helps.
Fix round time $t$ during this iteration of the \term{while} loop. Let $\IndPadded$, $\IndExplore$, $\IndExploit$ be the indicator variables for which phase this round is in. Let $\mF$ be the sigma-algebra generated by the conditional expectations $\widetilde{\mu}_1 \LDOTS \widetilde{\mu}_{j-1}$ and the true value $\mu_j$.

We first observe that
    $\Pr\sbr{ \IndPadded\mid \mF}$
is a decreasing function of $\widetilde{\mu}_i$, for each $i<j$, and independent of $\mu_j$.  Indeed, $\IndPadded$ is determined by the event $\ZEROS_{j,N_0}$ and the (independent) choices in Line~\ref{line:algexplore}. The event $\ZEROS_{j,N_0}$ is independent of $\mu_j$, and decreasing in each $\tilde{\mu}_i$.

Fix an arm $i< j$. We want to prove the BIC property relative to arm $i$:

\begin{align}\label{eq:pf:lm:main-BIC-i}
\E\sbr{\Lambda_{i,j}}\geq 0,
\quad\text{where}\quad
\Lambda_{i,j} := (\mu_j-\mu_i)\cdot \ind{A_t=j}.
\end{align}
For the padded phase, we are similarly interested in
    $\padExpr := (\mu_j-\mu_i)\cdot \ind{\pi_j=j}$.

%\begin{align*}
%\mathbb E[(\mu_j-\mu_i)\cdot 1_{A_t=a_j}\cdot 1_{padded}]
%&=\mathbb E\left[ \mathbb E [(\mu_j-\mu_i)1_{A_t=a_j}|\mathcal F]\cdot \mathbb E[1_{padded}|\mathcal F]\right]\\
%&\geq \mathbb E[\mathbb E[(\mu_j-\mu_i)\cdot 1_{A_t=a_j}|\mathcal F]]\cdot \mathbb E[\mathbb E[1_{padded}|\mathcal F]]\\
%&=\mathbb E[(\mu_j-\mu_i)1_{A_t=a_j}]\cdot p_{j}\\
%&\geq \lambda p_{j}.
%\end{align*}

The $j$-correlation property allows us to apply the FKG inequality to
    $\E \sbr{ \padExpr\mid \mF}$
and
    $\E\sbr{ \IndPadded\mid \mF}$,
which we interpret as functions of $\mu_1 \LDOTS \mu_j$.
Indeed these functions are decreasing in each $\widetilde{\mu}_i$, $i<j$ and increasing in $\mu_j$. By reparametrizing we may say both functions are increasing in each $-\widetilde{\mu}_i$ and in $\mu_j$, which are jointly independent, and therefore that FKG implies non-negative correlation.

\ascomment{As stated, FKG requires each function to be monotone \emph{in the same direction} for all coordinates.}

\ascomment{The $j$-correlated property conditions on the data rather than on $\mF$, and treats the conditional expectation as a function of the posterior means, rather than $\mu_i$.}

\ascomment{The $j$-correlated property talks about monotonicity of $\ind{\pi_j=j}$, rather than that of $\padExpr$.}

\ascomment{In the equations below, we need to switch from $\Lambda_{ij}$ to $\padExpr$, don't we? Then we can use the padding property in the last step.}

\begin{align}
\E\sbr{ \Lambda_{i,j}\cdot \IndPadded}
    &= \E\sbr{ \padExpr\cdot \IndPadded} \\
    &=   \E\sbr{ \E [\padExpr\mid\mF]
        \;\cdot\; \E[\IndPadded\mid\mF]}
        &\EqComment{\ascomment{why??}}\\
    &\geq \E\sbr{ \E\sbr{\padExpr\mid\mF}}
        \;\cdot\; \E\sbr{\E\sbr{ \IndPadded\mid\mF}}
        & \EqComment{by FKG inequality}\\
    &=\E\sbr{ \padExpr} \cdot \E\sbr{\IndPadded} \\
    &\geq \padding\, p_{j}.
\end{align}
In the last step, we used the $(j,\padding)$-padded property:
    $\E\sbr{\Lambda^{\term{pad}}_{i,j} } \geq \padding$,
and the fact that
    $\E\sbr{\IndPadded} = p_j$.
The latter holds by the algorithm's specification and Invariant 2.
%In the second-to-last step we used the fact that $\E[\E[X|\mF]]=\E[X]$ for any random variable $X$.
Next,
\begin{align*}
\E\sbr{ \Lambda_{i,j}\cdot \IndPadded}
    &\geq \padding p_j\\
\E\sbr{ \Lambda_{i,j}\cdot \IndExplore}
    &\geq -\E[\IndExplore]\geq  -\padding\, p_j\\
\E\sbr{\Lambda_{i,j}\cdot \IndExploit}
    &\geq 0.
\end{align*}
Here the third inequality holds by definition of exploitation. Summing up all three, we derive \eqref{eq:pf:lm:main-BIC-i}.


Now fix an arm $i>j$. We just use the BIC property of policy $\pi_j$, since
the $(j,\padding)$-padded property does not help. We use the FKG inequality as above, replacing $\padding$ with $0$, so as to deduce that
    $\E\sbr{ \Lambda_{i,j}\cdot \IndPadded}\geq 0$.
Then, we observe that
    $\E\sbr{ \Lambda_{i,j}\cdot \IndExplore} \geq 0$,
because $\mu_j^0\geq \mu_i^0$.
Moreover, $\E[\Lambda_{i,j}\cdot \IndExploit]\geq 0$ by definition of exploitation. Summing up all three inequalities, we derive \eqref{eq:pf:lm:main-BIC-i}.
\end{proof}


Now, we show that a suitable policy $\pi_j$ exists, in terms of the following parameters:
\begin{align}
\padG &= \min_{j,\,q\in \Delta_{j-1}}\E\sbr{ \rbr{ \mu_j-\mu_q}_+ },
\quad \text{where }
    \mu_q := \textstyle  \sum_{i \in [K]} q_i\, \mu_i. \nonumber \\
\padN &=  \padC\, \padG^{-2}\, \log \rbr{\padG^{-1}},
    \label{eq:params-padded}
\end{align}
for large enough absolute constant $\padC$. In words, $\padG$ is the smallest ``expected advantage" of any arm $j$ over a convex combination of arms $i<j$. We merely guarantee existence of a policy via the minimax theorem, rather than specify how to compute it.


\begin{lemma}\label{lm:policy-existence}
For each arm $j\geq 2$ there exists a policy $\pi_j$ which is $(j,\padding,\padN)$-suitable,
for
 $\padding = \nicefrac{\padG}{10}$.
\end{lemma}
\begin{proof}[Proof Sketch]
Fix arm $j\geq 2$. Maximizing padding $\padding$ in \refeq{eq:padded-BIC-defn} is naturally expressed as a zero-sum game between a \emph{planner} who chooses a $(j,N)$-informed  policy $\pi_j$ and wishes to maximize the right-hand side of \eqref{eq:padded-BIC-defn}, and an \emph{agent} who chooses arm $i$; we call it the \emph{$(j,N)$-recommendation game}.%
\footnote{It is a finite game because there are only finitely many deterministic $(j,N)$-informed policies.}
 A policy $\pi_j$ is $(j,\padding)$-padded if and only if it is guaranteed payoff at least $\padding$ in this game. So, any maximin policy in this game is $(j,\padding)$-padded with $\padding = V_{j,N}$, where $V_{j,N}$ is the game value.

We connect the game value with $\padG$ via the minimax theorem, proving that
    $V_{j,N}\geq \padG/10$.
Indeed, using the minimax theorem and the linearity of expectation, we can write the game value as
\[ V_{j,N}
    = \min_{q\in \Delta_{j-1}} \quad
    \max_{\text{$(j,N)$-informed policies $\pi_j$}}\quad
    \E\sbr{ (\mu_j - \mu_q)\cdot \ind{\pi_j=j}}.
\]
If the policy $\pi_j$ knew the mean rewards $(\mu_1 \LDOTS \mu_j)$ exactly, it could recommend arm $j$ if and only if $\mu_j-\mu_q>0$. This would guarantee the minimax value of at least
    $G_j := \min_{q\in \Delta_{j-1}} \E\sbr{ \rbr{ \mu_j-\mu_q}_+ } $.
We show that for a large enough $N$ we can guarantee the minimax value of at least $\Omega(G_j)$. Specifically, for $N = \padN$ and any given distribution $q\in\Delta_{i-1}$ there exists a $(j,N)$-informed policy $\pi = \pi_{j,N}^{q}$ such that
\begin{align}\label{pf:lm:policy-existence-2}
 \E\sbr{ (\mu_j - \mu_q)\cdot \ind{\pi=j}}
        \geq \tfrac{1}{10}\cdot \E\sbr{ \rbr{ \mu_j-\mu_q}_+ }.
\end{align}
This policy is very simple: given the data (the first $N$ samples of each arm $i\leq j$), recommend arm $j$ if and only if its empirical reward on this data is larger than the expected reward of distribution $q$ on the same data. For every given realization of the mean rewards $(\mu_1 \LDOTS \mu_j)$, we use Chernoff Bounds to compare
    $(\mu_j - \mu_q)\cdot \ind{\pi=j}$ and $(\mu_j - \mu_q)_+$,
which implies \eqref{pf:lm:policy-existence-2}.

From here on, let us focus on the $(j,\padN)$-recommendation game. Use ``well-formed" as a shorthand for ``$(j,\padN)$-informed", so that planners strategies in the game are well-informed policies.

Thus, we have proved that there exists a well-formed policy $\pi_j$ that is $(j,\padding)$-padded, for $\padding = \padG/10$, even if we do not specify how to compute such policy. However, we are not done yet, as we also need such policy to be BIC and $j$-correlated given $\mG_{N,j}$.

Any finite two-player zero-sum game has a maximin strategy that is \emph{non-weakly-dominated}: not weakly dominated by any other mixed strategy for the max player. So, let us take a maximin policy $\pi^*$ that is non-weakly-dominated. One can prove that any such policy is $j$-correlated given $\mG_{N,j}$.

Finally, we extend $\pi^*$ to a BIC policy. When $\pi^*$ does \emph{not} recommend arm $j$, we choose an arm $i$ for exploitation, \ie to maximize
    $\E\sbr{ \mu_i \mid \asedit{\mG_{N,j}}}$.
The resulting policy is BIC, hence $(j,\padding,\padN)$-suitable.
\end{proof}

\noindent\textbf{Putting the pieces together.}
Let us formulate an end-to-end guarantee for the algorithm in terms of the appropriate parameters. Recall that we use $\padG,\padN$ from \eqref{eq:params-padded} to handle the ``padded phase".
Given \eqref{eq:cl:alg-obs:boot}, we define two more parameters to handle the ``bootstrapping phase":
\begin{align}\label{eq:params-boot}
\bootN &= \min \cbr{ N_0\in\N:\;
    \E\sbr{ \mu_j-\mu_i \mid \ZEROS_{j,N_0}} > 0
    \; \text{for all arms $i<j$}}. \\
\bootP &= \min_{\text{arms $j$}}
    \Pr\sbr{ \ZEROS_{j,\bootN} }.
\end{align}
In words, $\bootN$ is the smallest $N_0$ such that each arm $j$ is the best arm conditional on seeing $N_0$ initial samples from all arms $i<j$ that are all zeroes. Setting $N_0 = \bootN$ as we do in the theorem, $\bootP$ is the smallest phase-exploration probability after the bootstrapping phase.


\begin{restatable}{theorem}{goodalgo}
\label{thm:goodalgo}
Suppose algorithm \MainALG is run with parameters
    $N\geq \max(\bootN,\padN)$,
    $N_0 = \bootN$
and
    $\padding = \padG/10$.
Suppose each policy $\pi_i$ is $(j,\padding,N)$-suitable (such policies exist by Lemma~\ref{lm:policy-existence}). Then the algorithm is BIC and collects at least $N$ samples of each arm almost surely in time
\[ \RndsUB(N) = O\rbr{
    KN\;\padG^{-1}\; \log\rbr{\bootP^{-1}} }.\]
\end{restatable}

\xhdr{Significance.}
Theorem~\ref{thm:goodalgo} provides an explicit formula for the time horizon of \MainALG. This formula is an \emph{upper bound} on the the sample complexity in question. It is polynomially optimal and allows for lucid corollaries, as we discuss in Section~\ref{sec:LB}. Setting $N\geq N_{\TS}$, we collect enough data to bootstrap Thompson Sampling, as per Section~\ref{sec:TS}.

\xhdr{Implementation.}
\asedit{How to compute a suitable policy $\pi_j$ for Lemma~\ref{lm:policy-existence}? For $K=2$ arms, one can take a very simple policy $\pi_2$: given the first $N$ samples of both arms, recommend an arm with a larger empirical reward. (This idea can be extended to an arbitrary $K$, but the padding $\padding$ degrades exponentially in $K$; we omit the easy details.) We provide a computationally efficient implementation for Beta priors in Section~\ref{sec:ext}. However, we do not provide a computational implementation for the general case.}

\xhdr{Extension.}
\asedit{The algorithm is somewhat wasteful when $N\gg \max(\padN,\bootN)$. Indeed, only $\bootN$ rounds are needed for the bootstrapping phase to be BIC, and only $\padN$ rounds are needed for each iteration of the \term{while} loop to collect $\padN$ samples of arm $j$ almost surely. Once these samples are there, the remaining samples for arm $j$ can be collected more efficiently: indeed, one can directly randomize between an exploration phase and a padded phase. These modifications (see Algorithm~\ref{alg:pyramidtightfast} in Appendix~\ref{sec:improved-algo}) reduce the number of rounds needed to almost-surely collect $N$ samples of each arm to
\[ \RndsUBtwo(N) = O\rbr{
    K\;\padG^{-1}\; \rbr{\padN\,\log(\bootP^{-1}) + \bootN + N }}.\]
}

%prove that a very simple policy $\PiSimple_j$ suffices for Beta priors: given the $\padN$ samples of each arm $i\leq j$, recommend arm $j$ if its posterior mean reward is larger than the posterior mean reward averaged over all arms $i<j$; otherwise, choose an arm $i<j$ which maximizes  $\E[\; \mu_i \mid \PiSimple_j\neq j  \;]$.}


%Computing policies $\pi_j$ for \MainALG is not computationally efficient.

%We find policies $\pi_j$ in Lemma~\ref{lm:policy-existence} by solving a zero-sum game up to high precision. This is feasible via standard no-regret learning techniques
%\citep[\eg see Ch. 6 in][]{SchapireBoosting}. However, it is not computationally efficient because the game is very large.


%\subsection{Proof of Lemma~\ref{lm:policy-existence}}
%\label{sec:policy-existence}



==> sec-pyramid-2021-02-05.tex <==
\section{Collecting Initial Samples}
\label{sec:sampling}

We turn to a basic version of incentivized exploration: collect $N$ samples of each arm. We design a BIC algorithm, called \MainALG, which completes after a pre-determined number of rounds and collects $N$ samples of each arm almost surely.
(This is a desirable property as per Remark~\ref{rem:switch-time}.)
We bound the completion time in terms some parameters of the prior.


%how many rounds does it take to obtain $N$ samples from each arm almost surely? This is the ``waiting time" before switching to Thompson Sampling, as per Theorem~\ref{thm:TSsamples}, if  $N=N_{\TS}$.


%we now seek to efficiently acquire samples of each arm. We ask for a BIC algorithm which by a fixed time $T$ always achieves at least $\Nsamples$ samples of each arm, and seek to minimize $T$. For $\Nsamples\geq N_{\TS}$, this is the amount of waiting time before Thompson sampling can be implemented.


%Call a given arm \emph{explored} if it has been sampled at least $\Nsamples$ times.

We describe the algorithm on a high level, and then fill in the details.
We explore the arms in order of increasing index, \ie decreasing prior mean reward. A given arm $j$ is explored as follows. We partition time in phases of $N$ rounds each. Within a given phase, we recommend the same arm in all rounds. There are three options: ``pure exploration", when we always recommend arm $j$, ``pure exploitation", when we choose an arm with the largest posterior mean reward and recommend this arm throughout the phase, and a ``padded phase" which combines exploration and exploitation and enables an exponential boost in efficiency. In the ``padded phase", arm $j$ is recommended sufficiently often and for a sufficiently good reason so as to guarantee a stronger BIC property for arm $j$. This property is parameterized by a prior-dependent amount $\padding >0$. We think of this amount as ``padding", and leverage it to offset additional ``pure exploration".

%We guarantee that the ``pure exploration" phase is invoked almost surely

Algorithm~\ref{alg:pyramidtight} presents the algorithm with abstract parameters $N_0\leq N$ and $\padding>0$, and recommendation policies for the padded phase. Let us again focus on exploring a particular arm $j$. The three phases described above are interleaved in a somewhat intricate way. For bootstrapping, we have one phase in which we explore if the first $N_0$ samples of all previous arms $i<j$ returned zero rewards, and exploit otherwise. Then, we enter a \term{while} loop, where we grow the \emph{phase-exploration probability}: the probability that the ``pure exploration" phase for arm $j$ has been invoked. Once this happens, we permanently switch to the ``padded phase". Meanwhile, we randomize between ``pure exploitation" and ``pure exploitation" with predetermined probability. The latter is chosen to ensure that the phase-exploration probability is boosted by the factor $1+\padding$ at each iteration. This process continues until the phase-exploration probability reaches $1$.


% \begin{figure}[t]
% \SetKwFor{Loop}{loop}{}{end}

% \begin{algorithm2e}[H]\label{alg:pyramidtight}
% \caption{\MainALG}
% \SetAlgoLined\DontPrintSemicolon

% \textbf{Parameters:}
%     phase length $N$,
%     bootstrapping parameter $N_0\leq N$,
%     padding $\padding>0$.

% \textbf{Given:}
% recommendation policies $\pi_2 \LDOTS \pi_K$ for \PaddedPhase.

% \asedit{\ExplorePhase[1].}

% \For{each arm $j=\asedit{2}  \LDOTS K$}{ \label{line:algloop}
%     \tcp*[l]{Invariant 1: each arm $i<j$ has been sampled $\geq N$ times.}

%     \tcp*[f]{the bootstrapping phase}

%     Set $\ZEROS_{j,N_0} = \{\text{the first $N_0$ samples of each arm $i<j$ return reward $0$}\}$

%     \uIf{$\ZEROS_{j,N_0}$}{\ExplorePhase}
%         \uElse{\ExploitPhase.}



%     \tcp*[f]{grow the exploration probability}\\
%     Set $p_j=\Pr\sbr{\ZEROS_{j,N_0}}$.

%     \While{$p_j< 1$}{
%     \tcp*[l]{Invariant 2: $\Pr\sbr{\text{exploration phase has happened}}=p_j$}
%     \uIf{exploration phase has happened}{
%         \PaddedPhase: use policy $\pi_j$ for the next $N$ rounds
%         }
%     \uElse{
%     With probability $\min\rbr{1,\,\frac{p_j}{1-p_j}\cdot \padding}$, \ExplorePhase; \label{line:algexplore}
%     \\with the remaining probability: \ExploitPhase.
% }
% $p_j\leftarrow \min\rbr{1,\, p_j\, (1+\padding)}$
% }%end while
% } %end for
% \end{algorithm2e}
% \end{figure}

\newcommand{\happened}{exploration phase has happened\xspace}
\newcommand{\flag}{\term{flag}}
\newcommand{\invariant}[2]{\tcp*[l]{Invariant #1: #2.}} % \invariant{1}{blah}

\begin{figure}[H]
\SetKwFor{Loop}{loop}{}{end}

\begin{algorithm2e}[H]\label{alg:pyramidtight}
\caption{\MainALG}
\SetAlgoLined\DontPrintSemicolon

\textbf{Parameters:}
    phase length $N$,
    bootstrapping parameter $N_0\leq N$,
    padding $\padding>0$.

\textbf{Given:}
recommendation policies $\pi_2 \LDOTS \pi_K$ for \PaddedPhase.

\textbf{Initialize:} Sample arm $1$ $N$ times.

\For{each arm $j=2, 3  \LDOTS K$}{ \label{line:algloop}
    \invariant{1}{each arm $i<j$ has been sampled $\geq N$ times}

    \vspace{2mm}\tcp*[l]{Initialization}

    Event $\ZEROS_{j,N_0} = \{\text{the first $N_0$ samples of each arm $i<j$ return reward $0$}\}$. \\
    $p_j\leftarrow \Pr\sbr{\ZEROS_{j,N_0}}$.\\
    $\flag \leftarrow \term{false}$ 
    \tcp*[l]{$\flag = \text{true} \Rightarrow$ \happened}


    \vspace{2mm}\tcp*[l]{the bootstrapping phase}

    \uIf{$\ZEROS_{j,N_0}$}
        {\ExplorePhase \label{line:zeros1}}
    \uElse{
        \ExploitPhase. \label{line:nonzero1}}


    % \uIf{$\ZEROS_{j,N_0}$}{\PaddedPhase: use policy $\pi_j$ for the next $N$ rounds}
    %     \uElse{With probability $\min\rbr{1,\,\frac{p_j}{1-p_j}\cdot \padding}$, \ExplorePhase;
    %     \\ with the remaining probability; \ExploitPhase}

    \vspace{2mm}
    \tcp*[l]{the exploration-laundering phase}

    \uIf{\flag}{
        %Generate $N$ independent, artificial samples from arms $1,\dots,j-1$, using fake mean rewards sampled independently from the original priors. Let $\hat\mu_1,\dots,\hat\mu_{j-1}$ be the resulting conditional expectations for the fake means.\\

        %Use policy $\pi_j$ for the next $N$ rounds, applied to $(\hat\mu_1,\dots,\hat\mu_{j-1},\widetilde{\mu}_j)$, to decide whether to recommend arm $j$.\\

        %If not recommending arm $j$, do \ExploitPhase on $\widetilde{\mu}_1,\dots,\widetilde{\mu}_j$.\label{line:zeros2}\\

        \ExploitPhase

        With probability $\frac{\lambda p_j}{1-p_j}$:
         $\flag \leftarrow \term{false}$\label{line:makeindep} \tcp*[l]{forget exploration}
    }\uElse{
        With probability $\min\rbr{1,\,\frac{p_j}{1-p_j}\cdot \padding}$,\\
            \myTAB\ExplorePhase \label{line:alg1explorephase} \\
        With the remaining probability: \ExploitPhase.
    }

    Update $p_j\leftarrow \min(1,\frac{\lambda p_j}{1-p_j}).$

    \invariant{2}{$\Pr\sbr{\flag=\text{true} \mid \mG_{N,\,j-1}}=p_j$}

    \vspace{2mm}\tcp*[l]{main loop: grow the exploration probability}


    \While{$p_j< 1$}{
    \invariant{3}{$\Pr\sbr{\flag=\text{true}}=p_j$}

    \uIf{\flag}{
        \PaddedPhase: use policy $\pi_j$ for the next $N$ rounds
        }
    \uElse{
    With probability $\min\rbr{1,\,\frac{p_j}{1-p_j}\cdot \padding}$,\\
    \myTAB \ExplorePhase \label{line:algexplore}
    \\With the remaining probability: \ExploitPhase.
}
Update $p_j\leftarrow \min\rbr{1,\, p_j\, (1+\padding)}$
}%end while
} %end for
\end{algorithm2e}
\end{figure}


Let's make some observations that are immediate from the algorithm's specification.

\begin{claim}\label{cl:alg-obs}
The algorithm completes in
    $N+N\,\sum_{j=2}^K \ln_{1+\padding} \rbr{1/\Pr[\ZEROS_{j,N_0}]}$
rounds, and samples each arm at least $N$ times almost surely. Both invariants hold. The bootstrapping phase is BIC as long as
\begin{align}\label{eq:cl:alg-obs:boot}
 \E\sbr{ \mu_j-\mu_i \mid \ZEROS_{j,N_0} } \geq 0
    \quad \text{for all arms $i<j$}.
\end{align}
\end{claim}

The key is to specify what happens in the ``padded phase", and argue about  incentives that it creates.
The recommendation policy $\pi_j$ for a given arm $j$ needs to satisfy several properties in addition to being BIC.
\begin{itemize}

\item First and foremost, we require a stronger BIC property for arm $j$:
\begin{align}\label{eq:padded-BIC-defn}
\E\sbr{ (\mu_j - \mu_i)\cdot \ind{\pi_j=j}}\geq \padding
\quad\text{for each arm $i<j$}.
\end{align}
We say that policy $\pi_j$ is \emph{$(j,\padding)$-padded BIC} if \eqref{eq:padded-BIC-defn} holds, where $\lambda$ is the ``padding".
The left-hand side in \eqref{eq:padded-BIC-defn} is the expected loss for the $j\to i$ swap: the expected loss when one starts with policy $\pi_j$ and replaces arm $j$ with arm $i$ whenever arm $j$ is recommended. Note that we integrate over the event that arm $j$ being chosen, rather than condition on this event.

\item Second, we require $\pi_j$ to input only the first $N$ samples of each arm $i<j$; such policies are called $(j,N)$-informed. This property ensures that the algorithm has sufficient data to compute policy $\pi_j$.


\item \mscomment{Actually $j$-correlated is no longer needed in the main body. I thought it was needed because I forgot we are assuming $\pi_j$ is ordinary BIC, and was getting this BIC property as a corollary of being $j$-correlated. So I think we can delete this bullet point.} Third, we focus on the probability of recommending arm $j$ as a function of the posterior mean rewards
    $\widetilde{\mu}_i := \E\sbr{ \mu_i \mid \mathcal \mG_{N,j}}$,
    for each arm $i\leq j$.%
    \footnote{Recall that $\mG_{N,j}$ denotes the $\sigma$-algebra generated by the first $N$ samples of each arm $i\leq j$.}
    We posit that the conditional probability
        $\Pr\sbr{ \pi_j = j \mid \widetilde{\mu}_1 \LDOTS \widetilde{\mu}_j }$
    is monotonically  non-decreasing in $\widetilde{\mu}_j$ and monotonically non-increasing in $\widetilde{\mu}_i$ for each arm $i<j$. Such $\pi_j$ is callled \emph{$j$-correlated} given $\mG_{N,j}$.
    This is a natural property for a BIC recommendation policy that strives to explore arm $j$. We use it to apply the FKG inequality.

\end{itemize}
If policy $\pi_j$ is BIC and satisfies all three properties, it is called \emph{$(j,\padding,N)$-suitable}.


We show that these properties guarantee the \term{while} loop to be BIC. The main point is that the $(j,\lambda)$-padded property of policy $\pi_j$ compensates for the probability of new exploration.  The exploitation phase is only used to skip the round in a BIC way.%
\footnote{This is an interesting contrast with ``hidden exploration" \citep{ICexploration-ec15}, where the exploitation phase is used to offset exploration. We have little use for this, because the padded phase enables nearly as much additional exploration as possible.}
We rely on the FKG inequality to handle various technicalities.

\msedit{Crucially, all steps of the algorithm take a deterministic number of rounds. In particular, at any time $t$ we are in a non-random line of the algorithm, modulo If/Else statements.}

%A technical point is that being in the padded phase is not independent of the values $(\mu_i)_{i\leq j})$ due to the use of events $\ZEROS_{j,N_0}$ to start the exponential growth. Additionally, we must show that the BIC property continues to hold against the future arms $a_i$ for $i>j$. We handle both points by using the FKG inequality.

%We remark that our padded phase has the same functionality that the exploitation phase does in \cite{ICexploration-ec15}. By contrast, our exploitation phase is only used to skip the round in a BIC way. This is because by construction, our padded phase accounts for essentially as much additional exploration as possible, so in a sense all the value has been extracted out of the exploitation phase.


\newcommand{\IndPadded}{\indE{\term{padded}}}
\newcommand{\IndExplore}{\indE{\term{explore}}}
\newcommand{\IndExploit}{\indE{\term{exploit}}}
\newcommand{\IndFlag}{\indE{\term{exploreflag}}}

\newcommand{\padExpr}{\Lambda^{\term{pad}}_{i,j}}


\begin{lemma}\label{lm:main-BIC0}
Consider algorithm \MainALG with arbitrary parameters $N_0\leq N$ and $\padding>0$. Fix some arm $j\geq 2$. The bootstrapping and laundering phases are BIC as long as policy $\pi_j$ is $(j,\padding,N)$-suitable.
\end{lemma}

\begin{proof}

The bootstrapping phase is clearly BIC, since even the exploration phase is actually exploitation on the event $\ZEROS_{j,N_0}$. For the laundering phase, let $\IndFlag$, $\IndExplore$, $\IndExploit$ be the indicator variables for which type of phase is used. Fix an arm $i< j$. We want to prove the BIC property relative to arm $i$. Let $\Lambda_{i,j}=(\widetilde{\mu}_i-\widetilde{\mu}_j)\cdot 1_{A_t=j}.$ By definition of $\pi_j$ we have \[\mathbb E[(\widetilde{\mu}_j-\hat\mu_i)\cdot 1_{\pi_j=j}\cdot \IndFlag] \geq \lambda p_j.\]

Moreover for any $i<j$, the event $\IndFlag$ implies $\ZEROS_{j,N_0}$ which implies $\widetilde{\mu}_i\leq \hat{\mu}_i$. Therefore
\[\mathbb E[\Lambda_{i,j}\cdot \IndFlag] \geq \lambda p_j.\]

The only other possible non-exploitation step during the laundering phase comes from the exploration in line~\label{line:alg1explorephase}. This exploration happens with probability $\lambda p_j$ (because there is a $(1-p_j)$ probability to reach line~\ref{line:alg1explorephase} which cancels the denominator), hence: \[\mathbb E[(\widetilde{\mu}_j-\widetilde{\mu}_i)\cdot 1_{\pi_j=j}\cdot \IndExplore] \geq -\lambda p_j.\]

Finally in all exploitation phases, essentially by definition we have: \[\mathbb E[(\widetilde{\mu}_j-\widetilde{\mu}_i)\cdot 1_{\pi_j=j}\cdot \IndExploit] \geq 0.\]

We now add these three equations and observe that  $\IndFlag+\IndExplore+\IndExploit=1$ during the laundering phase, and also that $\mathbb E[(\widetilde{\mu}_j-\widetilde{\mu}_i)\cdot 1_{\pi_j=j}]=\mathbb E[(\mu_j-\mu_i)\cdot 1_{\pi_j=j}]$. We conclude the laundering phase is BIC against any arm $i<j$ when recommending arm $j$.

To verify the BIC property against arms $i>j$, we observe that $\mathbb E[\Lambda_{i,j}\cdot \IndFlag]\geq 0$ by the BIC property for $\pi_j$, since the fake data was only for arms $1,\dots,j-1$. On the other hand, the event that $A_t=j$ due to line~\ref{line:nonzero2} is independent of $\widetilde{\mu}_j$. Together these show the BIC property when recommending arm $j$ against arms $i>j$. Finally when recommending any arm $i\neq j$, the laundering phase must be exploiting, so we similarly conclude the BIC property holds in all cases.

\end{proof}


\begin{lemma}\label{lm:main-BIC}
Consider algorithm \MainALG with arbitrary parameters $N_0\leq N$ and $\padding>0$.
Fix some arm $j\geq 2$. Each iteration of the \term{while} loop is BIC as long as policy $\pi_j$ is $(j,\padding,N)$-suitable.
\end{lemma}



\begin{proof}
% \mscomment{The proof still has to use FKG a few times, so I think a proof outline may be better.}
% The main point is that if we use $\pi_j$ with probability $p_t$ on round $t$, then this ``by definition" cancels out the non-BICness of $\lambda p_t$ probability of exploration. The stipulation of being $j$-correlated allows us to use the FKG inequality to verify, for instance, that the fact that the initial exploitation phase was dependent on the previous arms only helps.





Consider a round occuring during the \term{while} loop for arm $j$. Let $\IndPadded$, $\IndExplore$, $\IndExploit$ be the indicator variables for which phase this round uses. Let $\mF$ be the sigma-algebra generated by the conditional expectations $\widetilde{\mu}_1 \LDOTS \widetilde{\mu}_{j}$.

We first observe that the events $\IndPadded$, $\IndExplore$, $\IndExploit$ are independent of $\mathcal F$. Indeed, at the time the \term{while} loop begins this is true thanks to line~\ref{line:makeindep}. Then throughout the \term{while} loop, the choice of exploration vs exploitation phase is also independent of $\mathcal F$, hence the claim.

By the independence just observed, we have:

\begin{align*}
\E\sbr{ \Lambda_{i,j}\cdot \IndPadded}
    &\geq  \padding p_j\\
\E\sbr{ \Lambda_{i,j}\cdot \IndExplore}
    &\geq -\E[\IndExplore]\geq  -\padding\, p_j\\
\E\sbr{\Lambda_{i,j}\cdot \IndExploit}
    &\geq 0.
\end{align*}

% For the padded phase, we are similarly interested in
%     $\padExpr := (\mu_j-\mu_i)\cdot \ind{\pi_j=j}$.

%\begin{align*}
%\mathbb E[(\mu_j-\mu_i)\cdot 1_{A_t=a_j}\cdot 1_{padded}]
%&=\mathbb E\left[ \mathbb E [(\mu_j-\mu_i)1_{A_t=a_j}|\mathcal F]\cdot \mathbb E[1_{padded}|\mathcal F]\right]\\
%&\geq \mathbb E[\mathbb E[(\mu_j-\mu_i)\cdot 1_{A_t=a_j}|\mathcal F]]\cdot \mathbb E[\mathbb E[1_{padded}|\mathcal F]]\\
%&=\mathbb E[(\mu_j-\mu_i)1_{A_t=a_j}]\cdot p_{j}\\
%&\geq \lambda p_{j}.
%\end{align*}

% The $j$-correlation property allows us to apply the FKG inequality to
%     $\E \sbr{ \padExpr\mid \mF}$
% and
%     $\E\sbr{ \IndPadded\mid \mF}$,
% which we interpret as functions of $\mu_1 \LDOTS \mu_j$.
% Indeed these functions are decreasing in each $\widetilde{\mu}_i$, $i<j$ and increasing in $\mu_j$. By reparametrizing we may say both functions are increasing in each $-\widetilde{\mu}_i$ and in $\mu_j$, which are jointly independent, and therefore that FKG implies non-negative correlation.

% \ascomment{As stated, FKG requires each function to be monotone \emph{in the same direction} for all coordinates.} Fixed this.

% \ascomment{The $j$-correlated property conditions on the data rather than on $\mF$, and treats the conditional expectation as a function of the posterior means, rather than $\mu_i$.}

% \ascomment{The $j$-correlated property talks about monotonicity of $\ind{\pi_j=j}$, rather than that of $\padExpr$.}

% \ascomment{In the equations below, we need to switch from $\Lambda_{ij}$ to $\padExpr$, don't we? Then we can use the padding property in the last step.}

% \begin{align*}
% \E\sbr{ \Lambda_{i,j}\cdot \IndPadded}
%     &= \E\sbr{ \padExpr\cdot \IndPadded} \\
%     &=   \E\sbr{ \E [\padExpr\mid\mF]
%         \;\cdot\; \E[\IndPadded\mid\mF]}
%         &\EqComment{\ascomment{why??}}\\
%     &\geq \E\sbr{ \E\sbr{\padExpr\mid\mF}}
%         \;\cdot\; \E\sbr{\E\sbr{ \IndPadded\mid\mF}}
%         & \EqComment{by FKG inequality}\\
%     &=\E\sbr{ \padExpr} \cdot \E\sbr{\IndPadded} \\
%     &\geq \padding\, p_{j}.
% \end{align*}
% In the last step, we used the $(j,\padding)$-padded property:
%     $\E\sbr{\Lambda^{\term{pad}}_{i,j} } \geq \padding$,
% and the fact that
%     $\E\sbr{\IndPadded} = p_j$.
% The latter holds by the algorithm's specification and Invariant 2.
% %In the second-to-last step we used the fact that $\E[\E[X|\mF]]=\E[X]$ for any random variable $X$.
% Next,
% \begin{align*}
% \E\sbr{ \Lambda_{i,j}\cdot \IndPadded}
%     &\geq \padding p_j\\
% \E\sbr{ \Lambda_{i,j}\cdot \IndExplore}
%     &\geq -\E[\IndExplore]\geq  -\padding\, p_j\\
% \E\sbr{\Lambda_{i,j}\cdot \IndExploit}
%     &\geq 0.
% \end{align*}
% Here the third inequality holds by definition of exploitation. Summing up all three, we derive \eqref{eq:pf:lm:main-BIC-i}.


When $i>j$, recommending arm $j$ is BIC against arm $i$ due to the ordinary BIC property which implies $\E\sbr{ \Lambda_{i,j}\cdot \IndPadded}\geq 0$, and the fact $\mu_j^0\geq \mu_i^0$ which implies $\E\sbr{ \Lambda_{i,j}\cdot \IndExplore}\geq 0$. Hence we obtain the same $3$ equations as just above, but with $\lambda= 0$. Finally when recommending an arm $i\neq j$ we are again only exploiting, so the proof that this is BIC is again similar to the previous lemma.



%     $\E\sbr{ \Lambda_{i,j}\cdot \IndPadded}\geq 0$.
% Then, we observe that
%     $\E\sbr{ \Lambda_{i,j}\cdot \IndExplore} \geq 0$,
% because $\mu_j^0\geq \mu_i^0$.
% Moreover, $\E[\Lambda_{i,j}\cdot \IndExploit]\geq 0$ by definition of exploitation. Summing up all three inequalities, we derive \eqref{eq:pf:lm:main-BIC-i}.
\end{proof}


Now, we show that a suitable policy $\pi_j$ exists, in terms of the following parameters:
\begin{align}
\padG &= \min_{j,\,q\in \Delta_{j-1}}\E\sbr{ \rbr{ \mu_j-\mu_q}_+ },
\quad \text{where }
    \mu_q := \textstyle  \sum_{i \in [K]} q_i\, \mu_i. \nonumber \\
\padN &=  \padC\, \padG^{-2}\, \log \rbr{\padG^{-1}},
    \label{eq:params-padded}
\end{align}
for large enough absolute constant $\padC$. In words, $\padG$ is the smallest ``expected advantage" of any arm $j$ over a convex combination of arms $i<j$. We merely guarantee existence of a policy via the minimax theorem, rather than specify how to compute it.


\begin{lemma}\label{lm:policy-existence}
For each arm $j\geq 2$ there exists a policy $\pi_j$ which is $(j,\padding,\padN)$-suitable,
for
 $\padding = \nicefrac{\padG}{10}$.
\end{lemma}
\begin{proof}[Proof Sketch]
Fix arm $j\geq 2$. Maximizing padding $\padding$ in \refeq{eq:padded-BIC-defn} is naturally expressed as a zero-sum game between a \emph{planner} who chooses a $(j,N)$-informed  policy $\pi_j$ and wishes to maximize the right-hand side of \eqref{eq:padded-BIC-defn}, and an \emph{agent} who chooses arm $i$; we call it the \emph{$(j,N)$-recommendation game}.%
\footnote{It is a finite game because there are only finitely many deterministic $(j,N)$-informed policies.}
 A policy $\pi_j$ is $(j,\padding)$-padded if and only if it is guaranteed payoff at least $\padding$ in this game. So, any maximin policy in this game is $(j,\padding)$-padded with $\padding = V_{j,N}$, where $V_{j,N}$ is the game value.

We connect the game value with $\padG$ via the minimax theorem, proving that
    $V_{j,N}\geq \padG/10$.
Indeed, using the minimax theorem and the linearity of expectation, we can write the game value as
\[ V_{j,N}
    = \min_{q\in \Delta_{j-1}} \quad
    \max_{\text{$(j,N)$-informed policies $\pi_j$}}\quad
    \E\sbr{ (\mu_j - \mu_q)\cdot \ind{\pi_j=j}}.
\]
If the policy $\pi_j$ knew the mean rewards $(\mu_1 \LDOTS \mu_j)$ exactly, it could recommend arm $j$ if and only if $\mu_j-\mu_q>0$. This would guarantee the minimax value of at least
    $G_j := \min_{q\in \Delta_{j-1}} \E\sbr{ \rbr{ \mu_j-\mu_q}_+ } $.
We show that for a large enough $N$ we can guarantee the minimax value of at least $\Omega(G_j)$. Specifically, for $N = \padN$ and any given distribution $q\in\Delta_{i-1}$ there exists a $(j,N)$-informed policy $\pi = \pi_{j,N}^{q}$ such that
\begin{align}\label{pf:lm:policy-existence-2}
 \E\sbr{ (\mu_j - \mu_q)\cdot \ind{\pi=j}}
        \geq \tfrac{1}{10}\cdot \E\sbr{ \rbr{ \mu_j-\mu_q}_+ }.
\end{align}
This policy is very simple: given the data (the first $N$ samples of each arm $i\leq j$), recommend arm $j$ if and only if its empirical reward on this data is larger than the expected reward of distribution $q$ on the same data. For every given realization of the mean rewards $(\mu_1 \LDOTS \mu_j)$, we use Chernoff Bounds to compare
    $(\mu_j - \mu_q)\cdot \ind{\pi=j}$ and $(\mu_j - \mu_q)_+$,
which implies \eqref{pf:lm:policy-existence-2}.

From here on, let us focus on the $(j,\padN)$-recommendation game. Use ``well-formed" as a shorthand for ``$(j,\padN)$-informed", so that planners strategies in the game are well-informed policies.

Thus, we have proved that there exists a well-formed policy $\pi_j$ that is $(j,\padding)$-padded, for $\padding = \padG/10$, even if we do not specify how to compute such policy. However, we are not done yet, as we also need such policy to be BIC and $j$-correlated given $\mG_{N,j}$.

Any finite two-player zero-sum game has a maximin strategy that is \emph{non-weakly-dominated}: not weakly dominated by any other mixed strategy for the max player. So, let us take a maximin policy $\pi^*$ that is non-weakly-dominated. One can prove that any such policy is $j$-correlated given $\mG_{N,j}$.

Finally, we extend $\pi^*$ to a BIC policy. When $\pi^*$ does \emph{not} recommend arm $j$, we choose an arm $i$ for exploitation, \ie to maximize
    $\E\sbr{ \mu_i \mid \asedit{\mG_{N,j}}}$.
The resulting policy is BIC, hence $(j,\padding,\padN)$-suitable.
\end{proof}

\noindent\textbf{Putting the pieces together.}
Let us formulate an end-to-end guarantee for the algorithm in terms of the appropriate parameters. Recall that we use $\padG,\padN$ from \eqref{eq:params-padded} to handle the ``padded phase".
Given \eqref{eq:cl:alg-obs:boot}, we define two more parameters to handle the ``bootstrapping phase":
\begin{align}\label{eq:params-boot}
\bootN &= \min \cbr{ N_0\in\N:\;
    \E\sbr{ \mu_j-\mu_i \mid \ZEROS_{j,N_0}} > 0
    \; \text{for all arms $i<j$}}. \\
\bootP &= \min_{\text{arms $j$}}
    \Pr\sbr{ \ZEROS_{j,\bootN} }.
\end{align}
In words, $\bootN$ is the smallest $N_0$ such that each arm $j$ is the best arm conditional on seeing $N_0$ initial samples from all arms $i<j$ that are all zeroes. Setting $N_0 = \bootN$ as we do in the theorem, $\bootP$ is the smallest phase-exploration probability after the bootstrapping phase.


\begin{restatable}{theorem}{goodalgo}
\label{thm:goodalgo}
Suppose algorithm \MainALG is run with parameters
    $N\geq \max(\bootN,\padN)$,
    $N_0 = \bootN$
and
    $\padding = \padG/10$.
Suppose each policy $\pi_i$ is $(j,\padding,N)$-suitable (such policies exist by Lemma~\ref{lm:policy-existence}). Then the algorithm is BIC and collects at least $N$ samples of each arm almost surely in time
\[ \RndsUB(N) = O\rbr{
    KN\;\padG^{-1}\; \log\rbr{\bootP^{-1}} }.\]
\end{restatable}

\xhdr{Significance.}
Theorem~\ref{thm:goodalgo} provides an explicit formula for the time horizon of \MainALG. This formula is an \emph{upper bound} on the the sample complexity in question. It is polynomially optimal and allows for lucid corollaries, as we discuss in Section~\ref{sec:LB}. Setting $N\geq N_{\TS}$, we collect enough data to bootstrap Thompson Sampling, as per Section~\ref{sec:TS}.

\xhdr{Implementation.}
How to compute a suitable policy $\pi_j$ for Lemma~\ref{lm:policy-existence}? For $K=2$ arms, one can take a very simple policy $\pi_2$: given the first $N$ samples of both arms, recommend an arm with a larger empirical reward. (This idea can be extended to an arbitrary $K$, but the padding $\padding$ degrades exponentially in $K$; we omit the easy details.) We provide a computationally efficient implementation for Beta priors in Section~\ref{sec:ext}. However, we do not provide a computational implementation for the general case.

\xhdr{Extension.}
The algorithm is somewhat wasteful when $N\gg \max(\padN,\bootN)$. Indeed, only $\bootN$ rounds are needed for the bootstrapping phase to be BIC, and only $\padN$ rounds are needed for each iteration of the \term{while} loop to collect $\padN$ samples of arm $j$ almost surely. Once these samples are there, the remaining samples for arm $j$ can be collected more efficiently: indeed, one can directly randomize between an exploration phase and a padded phase. These modifications (see Algorithm~\ref{alg:pyramidtightfast} in Appendix~\ref{sec:improved-algo}) reduce the number of rounds needed to almost-surely collect $N$ samples of each arm to
\[ \RndsUBtwo(N) = O\rbr{
    K\;\padG^{-1}\; \rbr{\padN\,\log(\bootP^{-1}) + \bootN + N }}.\]

%prove that a very simple policy $\PiSimple_j$ suffices for Beta priors: given the $\padN$ samples of each arm $i\leq j$, recommend arm $j$ if its posterior mean reward is larger than the posterior mean reward averaged over all arms $i<j$; otherwise, choose an arm $i<j$ which maximizes  $\E[\; \mu_i \mid \PiSimple_j\neq j  \;]$.}


%Computing policies $\pi_j$ for \MainALG is not computationally efficient.

%We find policies $\pi_j$ in Lemma~\ref{lm:policy-existence} by solving a zero-sum game up to high precision. This is feasible via standard no-regret learning techniques
%\citep[\eg see Ch. 6 in][]{SchapireBoosting}. However, it is not computationally efficient because the game is very large.


%\subsection{Proof of Lemma~\ref{lm:policy-existence}}
%\label{sec:policy-existence}



==> sec-pyramid-2021-02-06.tex <==
\section{Collecting Initial Samples}
\label{sec:sampling}

We turn to a basic version of incentivized exploration: collect $N$ samples of each arm. We design a BIC algorithm, called \MainALG, which completes after a pre-determined number of rounds and collects $N$ samples of each arm almost surely.
(This is a desirable property as per Remark~\ref{rem:switch-time}.)
We bound the completion time in terms some parameters of the prior.


%how many rounds does it take to obtain $N$ samples from each arm almost surely? This is the ``waiting time" before switching to Thompson Sampling, as per Theorem~\ref{thm:TSsamples}, if  $N=N_{\TS}$.


%we now seek to efficiently acquire samples of each arm. We ask for a BIC algorithm which by a fixed time $T$ always achieves at least $\Nsamples$ samples of each arm, and seek to minimize $T$. For $\Nsamples\geq N_{\TS}$, this is the amount of waiting time before Thompson sampling can be implemented.


%Call a given arm \emph{explored} if it has been sampled at least $\Nsamples$ times.

We describe the algorithm on a high level, and then fill in the details.
We explore the arms in order of increasing index $j$, \ie in the order of decreasing prior mean reward. A given arm $j$ is explored as follows. We partition time in phases of $N$ rounds each, where $N$ is a parameter. Within a given phase, we recommend the same arm in all rounds. There are three types of phases:
\begin{OneLiners}
\item \emph{Exploration phase}, when we always recommend arm $j$.
\item \asedit{\emph{$L$-exploitation phase}, when we choose an arm with the largest posterior mean reward given some data, and recommend this arm throughout the phase. The data consists of the first $\min(L,L_i)$ samples of each arm $i$, where $L_i$ is the number of samples of this arm that are available before the phase starts.}
\item \emph{Padded phase}, which combines exploration and exploitation. We recommend arm $j$ sufficiently often and for a sufficiently good reason so as to guarantee a stronger BIC property for arm $j$. This property is parameterized by a prior-dependent amount $\padding >0$. We think of this amount as ``padding", and leverage it to offset additional ``pure exploration".

\end{OneLiners}

%We guarantee that the ``pure exploration" phase is invoked almost surely

Algorithm~\ref{alg:pyramidtight} presents the algorithm with abstract parameters $N_0\leq N$ and $\padding>0$, and recommendation policies for the padded phase. Let us again focus on exploring a particular arm $j$. The three phases described above are interleaved in a somewhat intricate way. For bootstrapping, we have one phase in which we explore if the first $N_0$ samples of all previous arms $i<j$ returned zero rewards, and exploit otherwise. Then, we enter a \term{while} loop, where we grow the \emph{phase-exploration probability}: the probability that the ``pure exploration" phase for arm $j$ has been invoked. Once this happens, we permanently switch to the ``padded phase". Meanwhile, we randomize between ``pure exploitation" and ``pure exploitation" with predetermined probability. The latter is chosen to ensure that the phase-exploration probability is boosted by the factor $1+\padding$ at each iteration. This process continues until the phase-exploration probability reaches $1$.


% \begin{figure}[t]
% \SetKwFor{Loop}{loop}{}{end}

% \begin{algorithm2e}[H]\label{alg:pyramidtight}
% \caption{\MainALG}
% \SetAlgoLined\DontPrintSemicolon

% \textbf{Parameters:}
%     phase length $N$,
%     bootstrapping parameter $N_0\leq N$,
%     padding $\padding>0$.

% \textbf{Given:}
% recommendation policies $\pi_2 \LDOTS \pi_K$ for \PaddedPhase.

% \asedit{\ExplorePhase[1].}

% \For{each arm $j=\asedit{2}  \LDOTS K$}{ \label{line:algloop}
%     \tcp*[l]{Invariant 1: each arm $i<j$ has been sampled $\geq N$ times.}

%     \tcp*[f]{the bootstrapping phase}

%     Set $\ZEROS_{j,N_0} = \{\text{the first $N_0$ samples of each arm $i<j$ return reward $0$}\}$

%     \uIf{$\ZEROS_{j,N_0}$}{\ExplorePhase}
%         \uElse{\ExploitPhase.}



%     \tcp*[f]{grow the exploration probability}\\
%     Set $p_j=\Pr\sbr{\ZEROS_{j,N_0}}$.

%     \While{$p_j< 1$}{
%     \tcp*[l]{Invariant 2: $\Pr\sbr{\text{exploration phase has happened}}=p_j$}
%     \uIf{exploration phase has happened}{
%         \PaddedPhase: use policy $\pi_j$ for the next $N$ rounds
%         }
%     \uElse{
%     With probability $\min\rbr{1,\,\frac{p_j}{1-p_j}\cdot \padding}$, \ExplorePhase; \label{line:algexplore}
%     \\with the remaining probability: \ExploitPhase.
% }
% $p_j\leftarrow \min\rbr{1,\, p_j\, (1+\padding)}$
% }%end while
% } %end for
% \end{algorithm2e}
% \end{figure}

\newcommand{\happened}{exploration phase has happened\xspace}
\newcommand{\flag}{\term{flag}}
\newcommand{\invariant}[2]{\tcp*[l]{\textcolor{blue}{Invariant #1: #2.}}} % \invariant{1}{blah}

\begin{figure}[H]
\SetKwFor{Loop}{loop}{}{end}

\begin{algorithm2e}[H]\label{alg:pyramidtight}
\caption{\MainALG}
\SetAlgoLined\DontPrintSemicolon

\textbf{Parameters:}
    phase length $N$,
    bootstrapping parameter $N_0\leq N$,
    padding $\padding>0$.

\textbf{Given:}
recommendation policies $\pi_2 \LDOTS \pi_K$ for \PaddedPhase.

\textbf{Initialize:} \ExplorePhase[1]

\For{each arm $j=2, 3  \LDOTS K$}{ \label{line:algloop}
    \invariant{1}{each arm $i<j$ has been sampled $\geq N$ times}

    \vspace{1mm}\tcp*[l]{Bootstrapping: two phases}
    Event $\ZEROS_{j,N_0} = \cbr{ \text{the first $N_0$ samples of each arm $i<j$ return reward $0$}} $.\\
    $p_j\leftarrow \frac{\padding\cdot\Pr\sbr{\ZEROS_{j,N_0}}}{1+\padding\cdot\Pr\sbr{\ZEROS_{j,N_0}}}$.\\
    \ExploitPhase[N_0] \label{line:initialexploit}
    
    \textbf{with probability} $p_j$ \textbf{do}\\
        \myTAB\ExplorePhase \label{line:alg1explorephase} \\
    \textbf{else} \ExploitPhase
        

    \vspace{2mm}\tcp*[l]{main loop: grow the exploration probability}


    \While{$p_j< 1$}{
    \invariant{2}{$\Pr\sbr{\text{\happened}}=p_j$}

    \uIf{\happened}{
        \PaddedPhase: use policy $\pi_j$ for the next $N$ rounds
        }
    \uElse{
    \textbf{with probability} $\min\rbr{1,\,\frac{p_j}{1-p_j}\cdot \padding}$ \textbf{do}\\
    \myTAB \ExplorePhase \label{line:algexplore}\\
    \textbf{else} \ExploitPhase
}
Update $p_j\leftarrow \min\rbr{1,\, p_j\, (1+\padding)}$
}%end while
} %end for
\end{algorithm2e}
\end{figure}


Let's make some observations that are immediate from the algorithm's specification.

\begin{claim}\label{cl:alg-obs}
The algorithm completes in
    $N+N\,\sum_{j=2}^K \ln_{1+\padding} \rbr{\frac{1}{\lambda \Pr[\ZEROS_{j,N_0}]}}$
rounds, and samples each arm at least $N$ times almost surely. Both invariants hold. The bootstrapping phase is BIC as long as
\begin{align}\label{eq:cl:alg-obs:boot}
 \E\sbr{ \mu_j-\mu_i \mid \ZEROS_{j,N_0} } \geq 0
    \quad \text{for all arms $i<j$}.
\end{align}
\end{claim}

The key is to specify what happens in the ``padded phase", and argue about  incentives that it creates.
The recommendation policy $\pi_j$ for a given arm $j$ needs to satisfy several properties in addition to being BIC.
\begin{itemize}

\item First and foremost, we require a stronger BIC property for arm $j$:
\begin{align}\label{eq:padded-BIC-defn}
\E\sbr{ (\mu_j - \mu_i)\cdot \ind{\pi_j=j}}\geq \padding
\quad\text{for each arm $i<j$}.
\end{align}
We say that policy $\pi_j$ is \emph{$(j,\padding)$-padded BIC} if \eqref{eq:padded-BIC-defn} holds, where $\lambda$ is the ``padding".
The left-hand side in \eqref{eq:padded-BIC-defn} is the expected loss for the $j\to i$ swap: the expected loss when one starts with policy $\pi_j$ and replaces arm $j$ with arm $i$ whenever arm $j$ is recommended. Note that we integrate over the event that arm $j$ being chosen, rather than condition on this event.

\item Second, we require $\pi_j$ to input only the first $N$ samples of each arm $i<j$; such policies are called $(j,N)$-informed. This property ensures that the algorithm has sufficient data to compute policy $\pi_j$.


\item \mscomment{Actually $j$-correlated is no longer needed in the main body. I thought it was needed because I forgot we are assuming $\pi_j$ is ordinary BIC, and was getting this BIC property as a corollary of being $j$-correlated. So I think we can delete this bullet point.} Third, we focus on the probability of recommending arm $j$ as a function of the posterior mean rewards
    $\widetilde{\mu}_i := \E\sbr{ \mu_i \mid \mathcal \mG_{N,j}}$,
    for each arm $i\leq j$.%
    \footnote{Recall that $\mG_{N,j}$ denotes the $\sigma$-algebra generated by the first $N$ samples of each arm $i\leq j$.}
    We posit that the conditional probability
        $\Pr\sbr{ \pi_j = j \mid \widetilde{\mu}_1 \LDOTS \widetilde{\mu}_j }$
    is monotonically  non-decreasing in $\widetilde{\mu}_j$ and monotonically non-increasing in $\widetilde{\mu}_i$ for each arm $i<j$. Such $\pi_j$ is callled \emph{$j$-correlated} given $\mG_{N,j}$.
    This is a natural property for a BIC recommendation policy that strives to explore arm $j$. We use it to apply the FKG inequality.

\end{itemize}
If policy $\pi_j$ is BIC and satisfies all three properties, it is called \emph{$(j,\padding,N)$-suitable}.


We show that these properties guarantee the \term{while} loop to be BIC. The main point is that the $(j,\lambda)$-padded property of policy $\pi_j$ compensates for the probability of new exploration.  The exploitation phase is only used to skip the round in a BIC way.%
\footnote{This is an interesting contrast with ``hidden exploration" \citep{ICexploration-ec15}, where the exploitation phase is used to offset exploration. We have little use for this, because the padded phase enables nearly as much additional exploration as possible.}
We rely on the FKG inequality to handle various technicalities.

\msedit{Crucially, all steps of the algorithm take a deterministic number of rounds. In particular, at any time $t$ we are in a non-random line of the algorithm, modulo If/Else statements.}

%A technical point is that being in the padded phase is not independent of the values $(\mu_i)_{i\leq j})$ due to the use of events $\ZEROS_{j,N_0}$ to start the exponential growth. Additionally, we must show that the BIC property continues to hold against the future arms $a_i$ for $i>j$. We handle both points by using the FKG inequality.

%We remark that our padded phase has the same functionality that the exploitation phase does in \cite{ICexploration-ec15}. By contrast, our exploitation phase is only used to skip the round in a BIC way. This is because by construction, our padded phase accounts for essentially as much additional exploration as possible, so in a sense all the value has been extracted out of the exploitation phase.


\newcommand{\IndPadded}{\indE{\term{padded}}}
\newcommand{\IndExplore}{\indE{\term{explore}}}
\newcommand{\IndExploit}{\indE{\term{exploit}}}
\newcommand{\IndFlag}{\indE{\term{exploreflag}}}
\newcommand{\IndZero}{\indE{\ZEROS_{j,N_0}}}

\newcommand{\padExpr}{\Lambda^{\term{pad}}_{i,j}}


\begin{lemma}\label{lm:main-BIC0}
Consider algorithm \MainALG with arbitrary parameters $N_0\leq N$ and $\padding>0$. Fix some arm $j\geq 2$. The bootstrapping phases are BIC as long as policy $\pi_j$ is $(j,\padding,N)$-suitable.
\end{lemma}

\begin{proof}


Line~\ref{line:initialexploit} is BIC since even the exploration phase is actually exploitation on the event $\ZEROS_{j,N_0}$. For the next phase, is it clear that recommending any arm $i\neq j$ is BIC since it can only happen via exploitation. Hence we fix an arm $i\neq j$ and show that arm $j$ is BIC against arm $i$ in this phase, i.e. letting $\Lambda_{i,j}=(\mu_i-\mu_j)\cdot 1_{A_t=j}.$ we show

\[\mathbb E[\Lambda_{i,j}]\geq 0.\]

We break into cases depending on whether $i<j$ or $i>j$. In the easy case $i>j$, because the event of an exploration phase is independent of the mean rewards $(\mu_k)_{k\leq K}$ the BIC property is clear. In the main case $i<j$, the key claim is that 

\[\mathbb E[\Lambda_{i,j}\cdot \IndZero\cdot \IndExploit]\geq \frac{\padding\cdot\Pr\sbr{\ZEROS_{j,N_0}}}{1+\padding\cdot\Pr\sbr{\ZEROS_{j,N_0}}}.]\]

To see this we argue as follows. On the event $\ZEROS_{j,N_0}$, the conditional means $(\widetilde{\mu}_i)_{i<j}$ are as low as possible. As a result if we generate independent fake mean rewards $(\mu_i^{\term{fake}})_{i<j}$ and resulting posterior means $(\widetilde{\mu}_i^{\term{fake}})_{i<j}$ still based on $N$ samples,

The conditional expectation $\mathbb E[\Lambda_{i,j}|\ZEROS_{j,N_0}]$ 

Multiplying by the probability to exploit instead of explore finishes the proof of the claim.






% For the laundering phase, let $\IndFlag$, $\IndExplore$, $\IndExploit$ be the indicator variables for which type of phase is used. Fix an arm $i< j$. We want to prove the BIC property relative to arm $i$. Let $\Lambda_{i,j}=(\widetilde{\mu}_i-\widetilde{\mu}_j)\cdot 1_{A_t=j}.$ By definition of $\pi_j$ we have \[\mathbb E[(\widetilde{\mu}_j-\hat\mu_i)\cdot 1_{\pi_j=j}\cdot \IndFlag] \geq \lambda p_j.\]

% Moreover for any $i<j$, the event $\IndFlag$ implies $\ZEROS_{j,N_0}$ which implies $\widetilde{\mu}_i\leq \hat{\mu}_i$. Therefore
% \[\mathbb E[\Lambda_{i,j}\cdot \IndFlag] \geq \lambda p_j.\]

% The only other possible non-exploitation step during the laundering phase comes from the exploration in line~\label{line:alg1explorephase}. This exploration happens with probability $\lambda p_j$ (because there is a $(1-p_j)$ probability to reach line~\ref{line:alg1explorephase} which cancels the denominator), hence: \[\mathbb E[(\widetilde{\mu}_j-\widetilde{\mu}_i)\cdot 1_{\pi_j=j}\cdot \IndExplore] \geq -\lambda p_j.\]

% Finally in all exploitation phases, essentially by definition we have: \[\mathbb E[(\widetilde{\mu}_j-\widetilde{\mu}_i)\cdot 1_{\pi_j=j}\cdot \IndExploit] \geq 0.\]

% We now add these three equations and observe that  $\IndFlag+\IndExplore+\IndExploit=1$ during the laundering phase, and also that $\mathbb E[(\widetilde{\mu}_j-\widetilde{\mu}_i)\cdot 1_{\pi_j=j}]=\mathbb E[(\mu_j-\mu_i)\cdot 1_{\pi_j=j}]$. We conclude the laundering phase is BIC against any arm $i<j$ when recommending arm $j$.

% To verify the BIC property against arms $i>j$, we observe that $\mathbb E[\Lambda_{i,j}\cdot \IndFlag]\geq 0$ by the BIC property for $\pi_j$, since the fake data was only for arms $1,\dots,j-1$. On the other hand, the event that $A_t=j$ due to line~\ref{line:nonzero2} is independent of $\widetilde{\mu}_j$. Together these show the BIC property when recommending arm $j$ against arms $i>j$. Finally when recommending any arm $i\neq j$, the laundering phase must be exploiting, so we similarly conclude the BIC property holds in all cases.

\end{proof}


\begin{lemma}\label{lm:main-BIC}
Consider algorithm \MainALG with arbitrary parameters $N_0\leq N$ and $\padding>0$.
Fix some arm $j\geq 2$. Each iteration of the \term{while} loop is BIC as long as policy $\pi_j$ is $(j,\padding,N)$-suitable.
\end{lemma}



\begin{proof}
% \mscomment{The proof still has to use FKG a few times, so I think a proof outline may be better.}
% The main point is that if we use $\pi_j$ with probability $p_t$ on round $t$, then this ``by definition" cancels out the non-BICness of $\lambda p_t$ probability of exploration. The stipulation of being $j$-correlated allows us to use the FKG inequality to verify, for instance, that the fact that the initial exploitation phase was dependent on the previous arms only helps.





Consider a round occuring during the \term{while} loop for arm $j$. Let $\IndPadded$, $\IndExplore$, $\IndExploit$ be the indicator variables for which phase this round uses. Let $\mF$ be the sigma-algebra generated by the conditional expectations $\widetilde{\mu}_1 \LDOTS \widetilde{\mu}_{j}$.

We first observe that the events $\IndPadded$, $\IndExplore$, $\IndExploit$ are independent of $\mathcal F$. Indeed, at the time the \term{while} loop begins this is true thanks to line~\ref{line:makeindep}. Then throughout the \term{while} loop, the choice of exploration vs exploitation phase is also independent of $\mathcal F$, hence the claim.

By the independence just observed, we have:

\begin{align*}
\E\sbr{ \Lambda_{i,j}\cdot \IndPadded}
    &\geq  \padding p_j\\
\E\sbr{ \Lambda_{i,j}\cdot \IndExplore}
    &\geq -\E[\IndExplore]\geq  -\padding\, p_j\\
\E\sbr{\Lambda_{i,j}\cdot \IndExploit}
    &\geq 0.
\end{align*}

% For the padded phase, we are similarly interested in
%     $\padExpr := (\mu_j-\mu_i)\cdot \ind{\pi_j=j}$.

%\begin{align*}
%\mathbb E[(\mu_j-\mu_i)\cdot 1_{A_t=a_j}\cdot 1_{padded}]
%&=\mathbb E\left[ \mathbb E [(\mu_j-\mu_i)1_{A_t=a_j}|\mathcal F]\cdot \mathbb E[1_{padded}|\mathcal F]\right]\\
%&\geq \mathbb E[\mathbb E[(\mu_j-\mu_i)\cdot 1_{A_t=a_j}|\mathcal F]]\cdot \mathbb E[\mathbb E[1_{padded}|\mathcal F]]\\
%&=\mathbb E[(\mu_j-\mu_i)1_{A_t=a_j}]\cdot p_{j}\\
%&\geq \lambda p_{j}.
%\end{align*}

% The $j$-correlation property allows us to apply the FKG inequality to
%     $\E \sbr{ \padExpr\mid \mF}$
% and
%     $\E\sbr{ \IndPadded\mid \mF}$,
% which we interpret as functions of $\mu_1 \LDOTS \mu_j$.
% Indeed these functions are decreasing in each $\widetilde{\mu}_i$, $i<j$ and increasing in $\mu_j$. By reparametrizing we may say both functions are increasing in each $-\widetilde{\mu}_i$ and in $\mu_j$, which are jointly independent, and therefore that FKG implies non-negative correlation.

% \ascomment{As stated, FKG requires each function to be monotone \emph{in the same direction} for all coordinates.} Fixed this.

% \ascomment{The $j$-correlated property conditions on the data rather than on $\mF$, and treats the conditional expectation as a function of the posterior means, rather than $\mu_i$.}

% \ascomment{The $j$-correlated property talks about monotonicity of $\ind{\pi_j=j}$, rather than that of $\padExpr$.}

% \ascomment{In the equations below, we need to switch from $\Lambda_{ij}$ to $\padExpr$, don't we? Then we can use the padding property in the last step.}

% \begin{align*}
% \E\sbr{ \Lambda_{i,j}\cdot \IndPadded}
%     &= \E\sbr{ \padExpr\cdot \IndPadded} \\
%     &=   \E\sbr{ \E [\padExpr\mid\mF]
%         \;\cdot\; \E[\IndPadded\mid\mF]}
%         &\EqComment{\ascomment{why??}}\\
%     &\geq \E\sbr{ \E\sbr{\padExpr\mid\mF}}
%         \;\cdot\; \E\sbr{\E\sbr{ \IndPadded\mid\mF}}
%         & \EqComment{by FKG inequality}\\
%     &=\E\sbr{ \padExpr} \cdot \E\sbr{\IndPadded} \\
%     &\geq \padding\, p_{j}.
% \end{align*}
% In the last step, we used the $(j,\padding)$-padded property:
%     $\E\sbr{\Lambda^{\term{pad}}_{i,j} } \geq \padding$,
% and the fact that
%     $\E\sbr{\IndPadded} = p_j$.
% The latter holds by the algorithm's specification and Invariant 2.
% %In the second-to-last step we used the fact that $\E[\E[X|\mF]]=\E[X]$ for any random variable $X$.
% Next,
% \begin{align*}
% \E\sbr{ \Lambda_{i,j}\cdot \IndPadded}
%     &\geq \padding p_j\\
% \E\sbr{ \Lambda_{i,j}\cdot \IndExplore}
%     &\geq -\E[\IndExplore]\geq  -\padding\, p_j\\
% \E\sbr{\Lambda_{i,j}\cdot \IndExploit}
%     &\geq 0.
% \end{align*}
% Here the third inequality holds by definition of exploitation. Summing up all three, we derive \eqref{eq:pf:lm:main-BIC-i}.


When $i>j$, recommending arm $j$ is BIC against arm $i$ due to the ordinary BIC property which implies $\E\sbr{ \Lambda_{i,j}\cdot \IndPadded}\geq 0$, and the fact $\mu_j^0\geq \mu_i^0$ which implies $\E\sbr{ \Lambda_{i,j}\cdot \IndExplore}\geq 0$. Hence we obtain the same $3$ equations as just above, but with $\lambda= 0$. Finally when recommending an arm $i\neq j$ we are again only exploiting, so the proof that this is BIC is again similar to the previous lemma.



%     $\E\sbr{ \Lambda_{i,j}\cdot \IndPadded}\geq 0$.
% Then, we observe that
%     $\E\sbr{ \Lambda_{i,j}\cdot \IndExplore} \geq 0$,
% because $\mu_j^0\geq \mu_i^0$.
% Moreover, $\E[\Lambda_{i,j}\cdot \IndExploit]\geq 0$ by definition of exploitation. Summing up all three inequalities, we derive \eqref{eq:pf:lm:main-BIC-i}.
\end{proof}


Now, we show that a suitable policy $\pi_j$ exists, in terms of the following parameters:
\begin{align}
\padG &= \min_{j,\,q\in \Delta_{j-1}}\E\sbr{ \rbr{ \mu_j-\mu_q}_+ },
\quad \text{where }
    \mu_q := \textstyle  \sum_{i \in [K]} q_i\, \mu_i. \nonumber \\
\padN &=  \padC\, \padG^{-2}\, \log \rbr{\padG^{-1}},
    \label{eq:params-padded}
\end{align}
for large enough absolute constant $\padC$. In words, $\padG$ is the smallest ``expected advantage" of any arm $j$ over a convex combination of arms $i<j$. We merely guarantee existence of a policy via the minimax theorem, rather than specify how to compute it.


\begin{lemma}\label{lm:policy-existence}
For each arm $j\geq 2$ there exists a policy $\pi_j$ which is $(j,\padding,\padN)$-suitable,
for
 $\padding = \nicefrac{\padG}{10}$.
\end{lemma}
\begin{proof}[Proof Sketch]
Fix arm $j\geq 2$. Maximizing padding $\padding$ in \refeq{eq:padded-BIC-defn} is naturally expressed as a zero-sum game between a \emph{planner} who chooses a $(j,N)$-informed  policy $\pi_j$ and wishes to maximize the right-hand side of \eqref{eq:padded-BIC-defn}, and an \emph{agent} who chooses arm $i$; we call it the \emph{$(j,N)$-recommendation game}.%
\footnote{It is a finite game because there are only finitely many deterministic $(j,N)$-informed policies.}
 A policy $\pi_j$ is $(j,\padding)$-padded if and only if it is guaranteed payoff at least $\padding$ in this game. So, any maximin policy in this game is $(j,\padding)$-padded with $\padding = V_{j,N}$, where $V_{j,N}$ is the game value.

We connect the game value with $\padG$ via the minimax theorem, proving that
    $V_{j,N}\geq \padG/10$.
Indeed, using the minimax theorem and the linearity of expectation, we can write the game value as
\[ V_{j,N}
    = \min_{q\in \Delta_{j-1}} \quad
    \max_{\text{$(j,N)$-informed policies $\pi_j$}}\quad
    \E\sbr{ (\mu_j - \mu_q)\cdot \ind{\pi_j=j}}.
\]
If the policy $\pi_j$ knew the mean rewards $(\mu_1 \LDOTS \mu_j)$ exactly, it could recommend arm $j$ if and only if $\mu_j-\mu_q>0$. This would guarantee the minimax value of at least
    $G_j := \min_{q\in \Delta_{j-1}} \E\sbr{ \rbr{ \mu_j-\mu_q}_+ } $.
We show that for a large enough $N$ we can guarantee the minimax value of at least $\Omega(G_j)$. Specifically, for $N = \padN$ and any given distribution $q\in\Delta_{i-1}$ there exists a $(j,N)$-informed policy $\pi = \pi_{j,N}^{q}$ such that
\begin{align}\label{pf:lm:policy-existence-2}
 \E\sbr{ (\mu_j - \mu_q)\cdot \ind{\pi=j}}
        \geq \tfrac{1}{10}\cdot \E\sbr{ \rbr{ \mu_j-\mu_q}_+ }.
\end{align}
This policy is very simple: given the data (the first $N$ samples of each arm $i\leq j$), recommend arm $j$ if and only if its empirical reward on this data is larger than the expected reward of distribution $q$ on the same data. For every given realization of the mean rewards $(\mu_1 \LDOTS \mu_j)$, we use Chernoff Bounds to compare
    $(\mu_j - \mu_q)\cdot \ind{\pi=j}$ and $(\mu_j - \mu_q)_+$,
which implies \eqref{pf:lm:policy-existence-2}.

From here on, let us focus on the $(j,\padN)$-recommendation game. Use ``well-formed" as a shorthand for ``$(j,\padN)$-informed", so that planners strategies in the game are well-informed policies.

Thus, we have proved that there exists a well-formed policy $\pi_j$ that is $(j,\padding)$-padded, for $\padding = \padG/10$, even if we do not specify how to compute such policy. However, we are not done yet, as we also need such policy to be BIC and $j$-correlated given $\mG_{N,j}$.

Any finite two-player zero-sum game has a maximin strategy that is \emph{non-weakly-dominated}: not weakly dominated by any other mixed strategy for the max player. So, let us take a maximin policy $\pi^*$ that is non-weakly-dominated. One can prove that any such policy is $j$-correlated given $\mG_{N,j}$.

Finally, we extend $\pi^*$ to a BIC policy. When $\pi^*$ does \emph{not} recommend arm $j$, we choose an arm $i$ for exploitation, \ie to maximize
    $\E\sbr{ \mu_i \mid \asedit{\mG_{N,j}}}$.
The resulting policy is BIC, hence $(j,\padding,\padN)$-suitable.
\end{proof}

\noindent\textbf{Putting the pieces together.}
Let us formulate an end-to-end guarantee for the algorithm in terms of the appropriate parameters. Recall that we use $\padG,\padN$ from \eqref{eq:params-padded} to handle the ``padded phase".
Given \eqref{eq:cl:alg-obs:boot}, we define two more parameters to handle the ``bootstrapping phase":
\begin{align}\label{eq:params-boot}
\bootN &= \min \cbr{ N_0\in\N:\;
    \E\sbr{ \mu_j-\mu_i \mid \ZEROS_{j,N_0}} > 0
    \; \text{for all arms $i<j$}}. \\
\bootP &= \min_{\text{arms $j$}}
    \Pr\sbr{ \ZEROS_{j,\bootN} }.
\end{align}
In words, $\bootN$ is the smallest $N_0$ such that each arm $j$ is the best arm conditional on seeing $N_0$ initial samples from all arms $i<j$ that are all zeroes. Setting $N_0 = \bootN$ as we do in the theorem, $\bootP$ is the smallest phase-exploration probability after the bootstrapping phase.


\begin{restatable}{theorem}{goodalgo}
\label{thm:goodalgo}
Suppose algorithm \MainALG is run with parameters
    $N\geq \max(\bootN,\padN)$,
    $N_0 = \bootN$
and
    $\padding = \padG/10$.
Suppose each policy $\pi_i$ is $(j,\padding,N)$-suitable (such policies exist by Lemma~\ref{lm:policy-existence}). Then the algorithm is BIC and collects at least $N$ samples of each arm almost surely in time
\[ \RndsUB(N) = O\rbr{
    KN\;\padG^{-1}\; \log\rbr{\bootP^{-1}} }.\]
\end{restatable}

\xhdr{Significance.}
Theorem~\ref{thm:goodalgo} provides an explicit formula for the time horizon of \MainALG. This formula is an \emph{upper bound} on the the sample complexity in question. It is polynomially optimal and allows for lucid corollaries, as we discuss in Section~\ref{sec:LB}. Setting $N\geq N_{\TS}$, we collect enough data to bootstrap Thompson Sampling, as per Section~\ref{sec:TS}.

\xhdr{Implementation.}
How to compute a suitable policy $\pi_j$ for Lemma~\ref{lm:policy-existence}? For $K=2$ arms, one can take a very simple policy $\pi_2$: given the first $N$ samples of both arms, recommend an arm with a larger empirical reward. (This idea can be extended to an arbitrary $K$, but the padding $\padding$ degrades exponentially in $K$; we omit the easy details.) We provide a computationally efficient implementation for Beta priors in Section~\ref{sec:ext}. However, we do not provide a computational implementation for the general case.

\xhdr{Extension.}
The algorithm is somewhat wasteful when $N\gg \max(\padN,\bootN)$. Indeed, only $\bootN$ rounds are needed for the bootstrapping phase to be BIC, and only $\padN$ rounds are needed for each iteration of the \term{while} loop to collect $\padN$ samples of arm $j$ almost surely. Once these samples are there, the remaining samples for arm $j$ can be collected more efficiently: indeed, one can directly randomize between an exploration phase and a padded phase. These modifications (see Algorithm~\ref{alg:pyramidtightfast} in Appendix~\ref{sec:improved-algo}) reduce the number of rounds needed to almost-surely collect $N$ samples of each arm to
\[ \RndsUBtwo(N) = O\rbr{
    K\;\padG^{-1}\; \rbr{\padN\,\log(\bootP^{-1}) + \bootN + N }}.\]

%prove that a very simple policy $\PiSimple_j$ suffices for Beta priors: given the $\padN$ samples of each arm $i\leq j$, recommend arm $j$ if its posterior mean reward is larger than the posterior mean reward averaged over all arms $i<j$; otherwise, choose an arm $i<j$ which maximizes  $\E[\; \mu_i \mid \PiSimple_j\neq j  \;]$.}


%Computing policies $\pi_j$ for \MainALG is not computationally efficient.

%We find policies $\pi_j$ in Lemma~\ref{lm:policy-existence} by solving a zero-sum game up to high precision. This is feasible via standard no-regret learning techniques
%\citep[\eg see Ch. 6 in][]{SchapireBoosting}. However, it is not computationally efficient because the game is very large.


%\subsection{Proof of Lemma~\ref{lm:policy-existence}}
%\label{sec:policy-existence}



==> sec-related.tex <==
\section{Related work}

Our model of incentivized exploration was introduced in \citet{Kremer-JPE14}, who obtain an optimal policy for the special case of two arms and deterministic rewards.%
\footnote{The study of incentivized exploration, broadly construed, was initiated in
\citet{Kremer-JPE14,Che-13}.}
\cite{ICexploration-ec15-conf,ICexploration-ec15} consider the general case of stochastic multi-armed bandits and design BIC bandit algorithms with near-optimal regret rates, up to multiplicative factors that depend on the prior and the number of arms.%
\footnote{In fact, \cite{ICexploration-ec15-conf,ICexploration-ec15} obtain several results of this form: both for Bayesian regret and standard (frequentist) notion of regret, and both in the worst case and for each problem instance.}
Further, they obtain a general reduction from bandit algorithms to incentive-compatible ones, and derive several extensions: to correlated priors, partially known priors, contextual bandits, and bandits with auxiliary feedback. They also suggest a connection to participation incentives in medical trials. \citet{ICexplorationGames-ec16} focus on exploring all arms than can possibly be explored, and allow for misaligned incentives when the algorithm's reward is different from the agents' utility. Several other extensions were considered, under various simplifying assumptions: to repeated games
\citep{ICexplorationGames-ec16}, heterogenous agents \citep{Jieming-multitypes18},
social networks \citep{Bahar-ec16,Bahar-ec19},
and relaxed economic assumptions
\citep{Jieming-unbiased18}.  Several related but technically different models have been studied: with time-discounted utilities \citep{Bimpikis-exploration-ms17}, monetary incentives \citep{Frazier-ec14,Kempe-colt18}, and continuous information flow \citep{Che-13}. A textbook-like introduction to this line of work can be found in
\citet[Ch. 11,][]{slivkins-MABbook}.


Incentivized exploration is closely related to two important recent topics in theoretical economics.
Bayesian Persuasion
\citep[\eg][]{BergemannMorris-survey19,Kamenica-survey19}
studies, essentially, a single round of our model, where the ``principal" uses  information asymmetry to persuade the agent to take particular actions. Social learning
\citep[\eg][]{Horner-survey16,Golub-survey16}
studies various scenarios in which multiple strategic agents interact and learn over time in a shared environment. 

Exploration-exploitation problems with incentives issues arise in several other domains, such as dynamic pricing, auction design, and human computation. These problems substantially differ from one another (and from incentivized exploration), depending on who are the self-interested agents and what they control. A review of this literature can be found in Ch. 11.7 of
\citet{slivkins-MABbook}.


%Exploration-exploitation problems with incentives issues arise in several other scenarios that substantially differ from one another, depending on who are the self-interested agents and what they control: dynamic pricing
%    \citep[\eg][]{KleinbergL03,BZ09,BwK-focs13},
%dynamic auctions
%    \citep[\eg][]{AtheySegal-econometrica13,DynPivot-econometrica10,Kakade-pivot-or13},
%pay-per-click ad auctions
%    \citep[\eg][]{MechMAB-ec09,DevanurK09,Transform-ec10-jacm},
%human computation
%    \citep[\eg][]{RepeatedPA-ec14,Ghosh-itcs13,Krause-www13},
%and competition between firms
%    \citep[\eg][]{bergemann2000experimentation,keller2003price,CompetingBandits-merged}.

Exploration-exploitation tradeoff and multi-armed bandits received a huge amount of attention over the past few decades. The diverse and  evolving body of research has been summarized in several books:
    \citet{CesaBL-book},
    \citet{Bubeck-survey12},
    \citet{Gittins-book11},
    \citet{slivkins-MABbook}, and
    \citet{LS19bandit-book}.
Stochastic $K$-armed bandits
    \citep{Lai-Robbins-85,bandits-ucb1}
is a canonical ``basic" version of the problem, by now it is very well understood.

Thompson Sampling \citep{Thompson-1933} is a well-known bandit algorithm with much recent progress, see  \citet{TS-survey-FTML18} for background. Most relevantly, it enjoys Bayesian regret bounds which are optimal in the worst case
\citep{Russo-MathOR-14,bubeck2013prior} and improve for some ``nice" priors \citep{Russo-MathOR-14}. Also, it attains optimal ``frequentist" regret bounds if initialized with some simple priors
\citep{Shipra-colt12,Kaufmann-alt12,Shipra-aistats13}.


